Max-Margin Token Selection in Attention Mechanism

Attention mechanism is a central component of the transformer architecture which led to the phenomenal success of large language models. However, the theoretical principles underlying the attention mechanism are poorly understood, especially its nonconvex optimization dynamics. In this work, we explore the seminal softmax-attention model $f(\boldsymbol{X})=\langle \boldsymbol{Xv}, \texttt{softmax}(\boldsymbol{XWp})\rangle$, where $\boldsymbol{X}$ is the token sequence and $(\boldsymbol{v},\boldsymbol{W},\boldsymbol{p})$ are trainable parameters. We prove that running gradient descent on $\boldsymbol{p}$, or equivalently $\boldsymbol{W}$, converges in direction to a max-margin solution that separates $\textit{locally-optimal}$ tokens from non-optimal ones. This clearly formalizes attention as an optimal token selection mechanism. Remarkably, our results are applicable to general data and precisely characterize $\textit{optimality}$ of tokens in terms of the value embeddings $\boldsymbol{Xv}$ and problem geometry. We also provide a broader regularization path analysis that establishes the margin maximizing nature of attention even for nonlinear prediction heads. When optimizing $\boldsymbol{v}$ and $\boldsymbol{p}$ simultaneously with logistic loss, we identify conditions under which the regularization paths directionally converge to their respective hard-margin SVM solutions where $\boldsymbol{v}$ separates the input features based on their labels. Interestingly, the SVM formulation of $\boldsymbol{p}$ is influenced by the support vector geometry of $\boldsymbol{v}$. Finally, we verify our theoretical findings via numerical experiments and provide insights.

==> sec/add_fig.tex <==
    \begin{figure}[t]
    \centering
    \hspace{-15pt}
    \subfigure[The role of loss function]{
        \includegraphics[width=.33\columnwidth, trim={0 -.5cm 0 0}]{fig/diff_loss_func.pdf}
        \label{fig2:loss:sen}
        
    }%\caption{Global convergence}
    \hspace{-10pt}
    \subfigure[Evolution of softmax probability]{
        \includegraphics[width=.35\columnwidth, trim={0 .7cm 0 0}]{fig/sfx_probs.pdf}
        \label{fig:sfx prob}
    }%\caption{Convergence to global and local optima}
    \hspace{-10pt}
    \subfigure[Evolution of attention weights]{
        \includegraphics[width=.35\columnwidth, trim={0 .7cm 0 0}]{fig/p_norms.pdf}
        \label{fig:p norm}
    }
    \hspace{-15pt}
    \vspace{-2mm}
    \caption{
        \textbf{(a)} Global convergence of $\pb$ with different loss functions and scores. \textbf{(b)\&(c)} Evolution of softmax probability and attention weights when updating using normalized gradient or constant step size $\eta$.}
    \label{fig:add_fig}\vspace{-8pt}
    \end{figure}

==> sec/app-sec-nonlinear-head.tex <==
\section{Addendum to Section~\ref{sec nonlin}}
\input{supp/app_reg_path.tex}
\input{supp/app_local_path.tex}
\input{supp/app_local_path_iff.tex}

==> sec/app_global_reg_path.tex <==
\subsection{Proof of Theorem~\ref{lin det thm}}

==> sec/bc/GD_converge_04_20.tex <==
\section*{Attempt at Gradient Flow Analysis}

\begin{theorem}\label{lin flow thm} Consider the single input loss with label $Y=1$
\begin{align}
\Lc(\pb)=\exp(-\vb^\top\X^\top \sft{\Kb\pb}).\label{one loss}
\end{align}
Fix a vector $\vb\in\R^d$ and define
\[
\alpha = \arg\max_{k\in [T]}\vb^\top \x_{k},
\]
and suppose $\vb^\top (\x_{\alpha}-\x_{k})>0$ for all $k\neq \alpha$. \eqref{one loss} with exponential loss and gradient flow $\dpb_t=-\nabla \Lc(\pb_t)$ converges (after normalization) to the \eqref{svm} solution
\[
\ps=\arg\min_{\pb} \tn{\pb}\quad \text{such that}\quad  \pb^\top(\kb_{\alpha}-\kb_{k\neq \alpha})\geq 1.
\]
\end{theorem}
\begin{proof} Set $\Sbt=\sft{\Kb\pb_t}$ and $\Sbtt=\sfp{\Kb\pb_t}$. Define $\Gamma:=e^{-\vb^\top\x_\alpha}$ and $\gmax=\vb^\top\x_\alpha$ and $\ggap=\gmax-\max_{k\neq \alpha}\vb^\top\x_k$. Let us first write the gradient flow iterations
\[
\dpb_t=\X^\top \Sbtt\X\vb\cdot\exp(-\vb^\top \X^\top \Sbt).
\]
Here recall that $\sfp{\ab}=\diag{\sft{\ab}}-\sft{\ab}\sft{\ab}^\top$. Let us introduce the following notation
\begin{itemize}
\item $s_t=\sum_{k\neq \alpha}\Sbt_k$ (amount of irrelevance)
\item $\bgam=\X\vb$ (vector of scores)
\item $\obo=s_t^{-1}\sum_{k\neq \alpha}\Sbt_k\x_k$ (irrelevant mixture weighted by softmax)
\item $\agam=s_t^{-1}\sum_{k\neq \alpha}\bgam_k\Sbt_k$ (average score over irrelevant tokens).
\item $\obt=\agam^{-1}s_t^{-1}\sum_{k\neq \alpha}\bgam_k\Sbt_k\x_k$ (irrelevant mixture weighted by softmax and $\vb$)
\end{itemize}

With this notation, we can write
\begin{align}
\x(t)&:=\X^\top \Sbt=(1-s_t)\x_\alpha+s_t\obo\\
\xv(t)&:=\X^\top \diag{\Sbt}\X\vb=\gmax(1-s_t)\x_\alpha+\agam s_t\obt\\
\xw(t)&:=\X^\top \Sbt{\Sbt}^\top\X\vb=(\gmax(1-s_t)+\agam s_t)((1-s_t)\x_\alpha+s_t\obo)\\
\xv(t)-\xw(t)&:=(1-s_t)s_t(\gmax-\agam)\x_\alpha+s_t[\agam \obt-(\gmax(1-s_t)+\agam s_t)\obo]
\end{align}
%Also define $\xv(t)=\X^\top \diag{\sft{\Kb\pb_t}}\X\vb=\sum_{k\in [T]}\x_k$ and 
Now note that
\[
\X^\top \sfp{\Kb\pb_t}\X\vb=-\x(t)\x(t)^\top\vb
\]
\[
\dpb_t=\X^\top \sfp{\Kb\pb_t}\X\vb\cdot\exp(-\vb^\top \x(t)).
\]
We claim that $\pb_t=\Gamma\log(t)\cdot\ps+\rb_t$ where $\rb_t$ will be a small (sub-logarithmic) residual. Let us write 
\begin{align}
\drb_t&=\X^\top \sfp{\Kb\pb}\X\vb\cdot\exp(-\vb^\top \X^\top \sft{\Kb\pb})-\frac{\Gamma}{t}\ps.
\end{align}
\end{proof}


==> sec/bc/joint_04_08.tex <==
%We will use a semi-random model where contextual features are deterministic whereas label is stochastic.

\section{Implicit Bias with Linear Head and General Data}

In this section, we consider \eqref{patt} with linear head $\vb$ by focusing on the following optimization objective with logistic loss
\begin{align}
\Lc(\vb,\pb)=\frac{1}{n}\sum_{i=1}^n \ell(Y_i\cdot\vb^\top\X_i^\top \sft{\Kb_i\pb}).\label{lin det los}
\end{align}
\subsection{Convergence of Attention Weights $\pba$}
\begin{theorem}\label{lin det thm}\red{[SIMPLE BUT CORRECT]} Suppose classifier head $\vb\in\R^d$ is such that, for all inputs $i\in[n]$, it obeys
\[
Y_i\cdot\vb^\top \x_{i1}>|\vb^\top \x_{it}|,\quad\forall t\geq 2.
\]
Set $\Kb_i=\W^\top\X_i$. Consider \eqref{lin det los} with logistic loss and fixed $\vb$. This loss obeys conditions of Lemma \ref{label mix}. Thus, per Theorem \ref{meta thm}, the regularization path $\pb_R/R$ of \eqref{lin det los} converges to an \eqref{svm} solution $\pb^\svm/\tn{\pb^\svm}$.
\end{theorem}
A dataset that obeys Theorem \ref{lin det thm} is as follows when we set $\vb=\vstar$. 
\begin{example} \label{dominant first} Suppose for some $\vstar\in\R^d$: $\x_{i1}=Y_i\cdot\vstar$, $\tn{\x_{it}}<\tn{\vstar}$ for all $t\geq 2$, $i\in[n]$.
\end{example}

\subsection{Joint Convergence of Head $\vba$ and Attention Weights $\pba$}
Let us denote the mixed tokens by $\x_i^\pb=\X_i^\top\sft{\Kb_i\pb}$. Given these, we can train a linear classifier $\vb$. Since gradient-descent on logistic regression is biased towards SVM, we introduce the following problem
\begin{align}
\vs=\arg\min_{\vb\in\R^d}\tn{\vb}\quad\text{subject to}\quad Y_i\vb^\top\rb_i\geq 1.\label{svm-label2}\tag{$\vb$-SVM}
\end{align}
Above, we will refer to $1/\tn{\vb^\svm}$ as the \emph{label margin} to distinguish it from attention's \emph{context margin}. 

We will explore the joint implicit bias of $(\vb,\pb)$ when both contexts and labels are separable and optimizing $(\vb,\pb)$ can make logistic loss arbitrarily small. Here, our key assumption in quantifying joint implicit bias is that, if $(\x_i^\pb)_{i=1}^n$ contain irrelevant tokens, then, the label margin of \eqref{svm-label2} strictly shrinks. This is formalized below.
\begin{assumption} \label{label margin ass} Recall $\s_{\max}^\pb=\max_{i\in[n]} \sum_{t\in \Rcb_i} \ab_{it}^\pb$. Solving \eqref{svm-label2} with $\rb_i\gets \x_i^\pb$ results in at most $\Gamma-\nu\cdot\s_{\max}^\pb$ margin where $\Gamma>0$ is the maximum margin over all $\pb$ and $\nu>0$ is a scalar independent of $\pb$.
\end{assumption}


\begin{theorem} \red{[TO BE PROVEN]} Consider the joint optimization \eqref{lin det los} over $\vb,\pb$. Suppose there are token indices $(\alpha_i)_{i=1}^n$ as follows: Consider the max-margin classifier on $\rb_i:=\x_{i\alpha_i}$ with labels $Y_i$,
        \begin{align}
        \vs=\arg\min_{\vb\in\R^d}\tn{\vb}\quad\text{subject to}\quad Y_i\vb^\top\rb_i\geq 1.\label{svm-label}\tag{$\vb$-SVM}
        \end{align}
        Set the margin $\Gamma=1/\tn{\vs}$ and \red{suppose all training points $(\rb_i)_{i=1}^n$ are support vectors}\footnote{It is not clear if this assumption is needed. However, it is a realistic assumption for overparameterized learning [Muthukumar et al. JMLR'21]}. Suppose for all $t\neq \alpha_i$, we have that $\tn{\x_{ti}}<\Gamma$. Then, the joint regularization path of $(\vb,\pb)$ with radius $(r,R)$ converges as follows: $\pb_R/R$ converges to the solution of convex \eqref{svm} where $\Rc_i=\{\alpha_i\}$ is a singleton. $\vb_{r}/r$ converges to $\vs/\tn{\vs}$. 
        %with labels $(Y_i)_{i=1}^n$ and features $(\rb_i)_{i=1}^n$. 
    \end{theorem}
    \begin{proof} Set $\bar{\Gamma}=\sup_{t\neq \alpha_i} \tn{\x_{ti}}<\Gamma$. Suppose the claim is incorrect and either $\pb_R/R$ or $\vb_{r}/r$ fails to converge as $R,r$ grows. Set $\Xi=1/\tn{\ps}$, $\pbs=R\Xi\ps_R$ and $\vbs=r\Gamma\vs_r$. The high-level idea is obtaining a contradiction by proving that $(\vbs,\pbs)$ is a strictly better solution compared to $(\vb_r,\pb_R)$.
    
    Recall $s_i^\pb=1-\ab^{\pb}_{\alpha_i}$. Define $\bota_i^\pb=\frac{\sum_{t\neq \alpha_i}\ab_i^\pb \x_{it}}{\s_i^\pb}$ and note that $\tn{\bota_i^\pb}\leq \Gamma$.
    
    \begin{lemma}[Mixing irrelevant tokens decreases class margin] Given $\pb\in\R^d$, write $\x_i^\pb=\X_i^\top \sft{\Kb_i\pb}$. There exists a $\upsilon>0$ such that solving \eqref{svm-label} on $\x_i^\pb$ has cost at least $1/(\Gamma-\upsilon s_{\max}^\pb)$.
    \end{lemma}
    \begin{proof} Observe that $\x_i^\pb=(1-\s_i^\pb)\rb_i+\s_i^\pb \bota_i^\pb$. Now pick any classifier $\vb$ with $\tn{\vb}=\tn{\vs}$. We have that
    \begin{align}
    |\vb^\top \x_i^\pb|&\leq (1-\s_i^\pb)|\vb^\top \rb_i|+\s_i^\pb\tn{\vb^\top \bota_i^\pb}\\
    &\leq (1-\s_i^\pb)|\vb^\top \rb_i|+\s_i^\pb\bar{\Gamma}/\Gamma.
    \end{align}
    Taking infimum of both sides over $i$, using optimality of $\vs$, and using $\rb_i^\top\vs=1$ for all $i$, we find $\min_{i\in[n]}|\vb^\top \x_i^\pb|\leq(1-\s_i^\pb)+\s_i^\pb\bar{\Gamma}/\Gamma$. Normalizing the margin to $1$, the resulting SVM cost is at least 
    
    \end{proof}
    
    \noindent$\bullet$ \textbf{Case 1: $\pb_R/R$ does not converge.} Under this scenario there exists $\eps,\delta=\delta(\eps)>0$ such that there exists arbitrarily large $R$ with $\tn{\pb_R/R-\pbs/R}\geq \eps$ and margin induced by $\pb_R/R$ is at most $\Xi-\eps$. Recall the amount of irrelevance definition $\s_i^\pb=\sum_{t\neq \alpha_{i}} \ab_{it}^{\pb}$. Repeating the proof of Theorem \ref{meta thm} (specifically directly copying \eqref{smax difference}), we find that 
    \begin{align}\label{smax diff2}
        \log(\hat{s}_{\max})&\geq -(1-\gamma)(R/\Gamma)-\log T,\\
         -(R/\Gamma)-\log T\leq \log(s^\st_{\max})&\leq -(R/\Gamma)+\log T.
    \end{align}
    In words, $\pbs$ contains exponentially less irrelevance compared to $\pb_R$.
    
    \noindent$\bullet$ \textbf{Case 2: $\vb_r/r$ does not converge.} Then, there exists $\delta>0$ such that we can find arbitrarily large $r$ obeying $\tn{\vb_r/r-\vs/\tn{\vs}}\geq \delta$.
    \end{proof}

    

%under generic conditions, 
The following theorem shows that, if the label-margin induced by the first tokens $(\x_{i1})_{i=1}^n$ of each input is larger than the norm of the other tokens, then, mixing the other tokens strictly shrink the label-margin. Consequently, the first tokens naturally become the relevant set and all other tokens become irrelevant.
\begin{theorem} \red{[TO BE PROVEN]} Consider an SVM problem over the dataset $(Y_i,\rb_i)_{i=1}^n$

Suppose all inputs $\rb_i$ are support vectors (all constraints are tight!) and set the margin $\Gamma=1/\tn{\vs}$. Pick points $(\z_i)_{i=1}^n$ and $0\leq \alpha_i\leq 1$ with $\bar{\Gamma}=\sup_{i\in[n]}\tn{\z_i}<\Gamma$. Set $\rb'_i=(1-\alpha_i)\rb_i+\alpha_i\z_i$. Solving SVM over $(Y_i,\rb'_i)$ will lead to a margin of at most $\Gamma-\nu \max_{i\in[n]}\alpha_i$ for some $\nu>0$ (depending on $\Gamma-\bar{\Gamma}$).
\end{theorem}

Note that, the dataset described above is a generalization of Example \ref{dominant first}. For Example \ref{dominant first}, relevant tokens are simply $\rb_i=\pm \vstar$ and the SVM solution is $\vb^\svm=\vstar/\tn{\vstar}^2$.

\noindent\red{[This seems easy to prove if we just ask $\bar{\Gamma}<\eps\Gamma$ for some small $\eps>0$ (e.g.~by using perturbation argument around $\vs$)]}




==> sec/bc/joint_05_22.tex <==
%\input{sec/joint_fig.tex}
\section{Joint Convergence of Head $\vba$ and Attention Weights $\pba$}\label{sec joint}\vspace{-5pt}
%\textbf{Joint $\vb,\pb$ convergence:} 


In this section, we extend the preceding results to the general case of joint optimization of head $\vb$ and attention weights $\pb$ using a logistic loss function. To this aim, we focus on regularization path analysis, which involves solving \eqref{lin det losss} under ridge constraints and examining the solution trajectory as the constraints are relaxed. 

\noindent\textbf{High-level intuition.} Since the prediction is linear as a function of $\vb$, logistic regression in $\vb$ can exhibit its own implicit bias to a max-margin solution. Concretely, define the attention features $\x_i^\pb=\X_i^\top\sft{\Kb_i\pb}$ and define the dataset $\Sc^{\pb}=(Y_i,\x_i^\pb)$. If the dataset $\Sc^{\pb}$ is separable by $\vb$, then optimizing only $\vb$ will converge in the direction of the max-margin classifier by setting $\rb_i\gets \x^\pb_i$:
\begin{align}
\vs=\arg\min_{\vb\in\R^d}\tn{\vb}\quad\text{subject to}\quad Y_i\cdot\vb^\top\rb_i\geq 1.\label{svm-label2}\tag{CLS-SVM}
\end{align}
This motivates a clear question: \emph{Under what conditions, optimizing $\vb,\pb$ jointly will converge to their respective max-margin solutions?} We study this question in two steps. Loosely speaking, we will first assume that when solving \eqref{svm-label2}, all inputs $i\in[n]$ are also the support vectors. We will then relax this condition to uncover a more general implicit bias for $\pb$. Throughout we assume that the joint problem is separable and there exists $(\vb,\pb)$ asymptotically achieving zero training loss.


%The first stage assumes that  where the first phase provides the intuitive answer and second phase establishes a more refine.

%Let us denote the mixed tokens by $\x_i^\pb=\X_i^\top\sft{\Kb_i\pb}$. Given these, we can train a linear classifier $\vb$. Since gradient-descent on logistic regression is biased towards SVM, we introduce the following problem

%Above, we will refer to $1/\tn{\vb^\svm}$ as the \emph{label margin} to distinguish it from attention's \emph{context margin}. 
\vspace{-5pt}
\subsection{When all attention features are support vectors}\vspace{-3pt}
%We will explore the joint implicit bias of $(\vb,\pb)$ when both contexts and labels are separable and optimizing $(\vb,\pb)$ can make logistic loss arbitrarily small. Here,
%To keep notation concise, we assume first token of each input is the optimal choice. The assumption below formalizes this: We assume that, without losing generality,

%The choice of first tokens is for notational convenience and without losing generality. 
In \eqref{svm-label2}, define \emph{label margin} to be $1/\tn{\vb^\svm}$. Our first insight in quantifying joint implicit bias is that, optimal tokens admit a natural definition: Those that maximize the downstream label margin when selected. This is formalized below where we assume that: (1) selecting the token indices $\bal=(\alpha_i)_{i=1}^n$ from each input data achieves the largest label margin. (2) The optimality of the $\bal$ choice is strict in the sense that mixing other tokens will shrink the label margin in \eqref{svm-label2}.
%assumption in quantifying joint implicit bias is that, if $(\x_i^\pb)_{i=1}^n$ contain irrelevant tokens, then, the label margin of \eqref{svm-label2} strictly shrinks. 
\begin{assumption} \label{label margin ass} Let $\Gamma>0$ be the label margin when solving \eqref{svm-label2} with $\rb_i\gets \x_{i\alpha_i}$. There exists $\nu>0$ such that for all $\pb$, solving \eqref{svm-label2} with $\rb_i\gets \x_i^\pb$ results in a label margin of at most $\Gamma-\nu\cdot \max_{i\in[n]} (1-\s_{i\alpha_i})$ where $\s_i=\sft{\Kb_i\pb}$. 
\end{assumption}
\SO{Is above margin-shrinkage assumption implied by the statement: $\Gamma$ is the unique maximum achievable margin over all $\pb$ (and associated $\rb_i\gets\x_i^\pb$) choices. Essentially, how will the margin shrink in terms of $\max_{i\in[n]}(1-\s_{i\alpha_i})$?}
%\red{\begin{assumption} \label{margin ass better} Let $\Gamma>0$ be the label margin when solving \eqref{svm-label2} with $\rb_i\gets \x_{i\alpha_i}$. $\Gamma$ is the unique maximum margin over all $\pb$ (and associated $\s_i=\sft{\Kb_i\pb}$) choices.\end{assumption}}
%There exists $\nu>0$ such that for all $\pb$, solving \eqref{svm-label2} with $\rb_i\gets \x_i^\pb$ results in a label margin of at most $\Gamma-\nu\cdot \max_{i\in[n]} (1-\s_{i\alpha_i})$ where $\s_i=\sft{\Kb_i\pb}$. 
%A dataset that obeys Theorem \ref{lin det thm} is as follows when we set $\vb=\vstar$. 
%Note that, our choice of first tokens is for notational convenience and without losing generality. 
\noindent\textbf{Example:} To gain intuition, let us fix $\vstar\in\R^d$ and consider the dataset obeying $\x_{i1}=Y_i\cdot \vstar$ and $\tn{\x_{it}}<\tn{\vstar}$ for all $t\geq 2$ and all $i\in[n]$. For this dataset, we can choose $\alpha_i=1$, $\Gamma=\tn{\vstar}$ and $\nu=\tn{\vstar}-\sup_{i\in[n],t\geq 2}\tn{\x_{it}}$.
% maximize downstream margin

\begin{theorem}\label{thm:path:joint:vp} Consider the ridge-constrained solutions $(\vb_r,\pb_R)$ of \eqref{lin det losss} defined as
\[
\vb_r,\pb_R=\underset{\tn{\vb}\leq r,\tn{\pb}\leq R}{\arg\min}\Lc(\vb,\pb).
\]
Suppose Assumption \ref{label margin ass} holds for some $\Gamma,\nu>0$. As $r,R\rightarrow\infty$, the joint regularization path $(\vb_r,\pb_R)$ converges as follows: $\frac{\pb_R}{R}\rightarrow\frac{\ps}{\tn{\ps}}$ where $\ps$ is the solution of \eqref{attnsvm}. $\frac{\vb_{r}}{r}\rightarrow \frac{\vs}{\tn{\vs}}$ where $\vs$ is the solution of \eqref{svm-label2} with $\rb_i=\x_{i1}$. 
\end{theorem}

As further discussion, consider Figure \ref{fig2:allsvm} where we set $n=3,T=d=2$ and $\W=\text{Identity}$. All three inputs share the point $(0,0)$ which corresponds to their non-optimal tokens. The optimal tokens (denoted by $\star$) are all support vectors of the \eqref{svm-label2} since $\vs=[0,1]$ is the optimal classifier direction (blue color). Because of this, $\ps$ will separate optimal tokens from $(0,0)$ coordinate via \eqref{attnsvm} which results in the red direction (yellow and teal $\star$ are the support tokens).
%Set $\bar{\Gamma}=\sup_{t\neq \alpha_i} \tn{\x_{ti}}<\Gamma$. 

\input{sec/joint_fig.tex}
\vspace{-5pt}
\subsection{General solution when selecting one token per input}\vspace{-3pt}

%, and without losing generality, again assume $\alpha_i=1$
Can we relax Assumption \ref{label margin ass}, and if so, what is the resulting behavior? Consider the scenario where the optimal $\pb$ diverges to $\infty$ and ends up selecting one token per input. Suppose this $\pb$ selects some coordinates $\bal=(\alpha_i)_{i=1}^n$. Let $\Nc\subset[n]$ be the set of indices where the associated token $\x_{i\alpha_i}$ is \textbf{not} a support vector when solving \eqref{svm-label2}. Our intuition is as follows: Even if we slightly perturb this $\pb$ choice and mix other tokens $t\neq \alpha_i$ over the input set $\Nc\subset[n]$, since $\Nc$ is not support vector for \eqref{svm-label2}, we can preserve the label margin (by only preserving the support vectors $[n]-\Nc$). This means that $\pb$ may not have to enforce \emph{max-margin} constraint over inputs $i\in\Nc$, instead, it suffices to just select these tokens (asymptotically). This results in the following \textbf{relaxed SVM} problem:
\begin{align} 
\prr=\min_{\pb} \tn{\pb}\quad\text{such that}\quad \pb^\top (\kb_{i\alpha_i}-\kb_{it})\geq \begin{cases} 1\quad\text{for all}\quad t\neq \alpha_i,~i\in[n]-\Nc\\ 0\quad\text{for all}\quad t\neq \alpha_i,~i\in\Nc\end{cases}.\label{relax svm}
\end{align}
Here, $\pb^\top \x_{i\alpha_i}\geq 0$ corresponds to the \emph{selection} idea. Building on this intuition, the following theorem captures the generalized behavior of the joint regularization path.
%for some indices $(\alpha_i)_{i=1}^n$, 
%$\x^{\pb_R}_i:=\X_i^\top\sft{\Kb_i\pb_R}\rightarrow \x_{i\alpha_i}$
%Let $\eb_j$ be the $j$'th standard basis vector. 
\begin{theorem}\label{joint thm general} Consider the path of $(\vb_r,\pb_R)$ as $r,R\rightarrow\infty$ as in Theorem \ref{thm:path:joint:vp}. \red{Suppose $\sft{\Kb_i\pb_R}_{\alpha_i}\rightarrow 1$}, i.e., the tokens $(\alpha_i)_{i=1}^n$ are asymptotically selected. Then, $\vb_{r}/{r}\rightarrow \vs/\tn{\vs}$ where $\vs$ is the solution of \eqref{svm-label2} with $\rb_i=\x_{i\alpha_i}$, $\Nc$ is the set of non-support vectors for \eqref{svm-label2}, and $\frac{\pb_R}{R}\rightarrow\frac{\prr}{\tn{\prr}}$ where $\prr$ is the solution of \eqref{relax svm} with $\alpha_i$ choices.
\end{theorem}
\SO{Does $\sft{\Kb_i\pb_R}_{\alpha_i}\rightarrow 1$ above imply margin-shrinkage Assumption \ref{label margin ass} when we mix non-$\alpha_i$ tokens (over support vectors)? Otherwise, we need to add the sentence ``Suppose Assumption \ref{label margin ass} holds over the support vectors $[n]-\Nc$.''}
To illustrate this numerically, consider Figure \ref{fig2:nosvm} which modifies Figure \ref{fig2:allsvm} by pushing the yellow $\star$ to the northern position $(0.5,1.5)$. We still have $\vs=[0,1]$ however the yellow $\star$ is no longer a support vector of \eqref{svm-label2}. Thus, $\pb$ solves the relaxed problem which separates green and teal $\star$'s by enforcing the max-margin constraint on $\pb$ (which is the red direction). Instead, yellow $\star$ only needs to achieve positive correlation with $\pb$ (unlike Figure \ref{fig2:nosvm} where it dictates the direction).

%\begin{theorem}\label{joint thm general} Consider the path of $(\vb_r,\pb_R)$ as $r,R\rightarrow\infty$ as in Theorem \ref{thm:path:joint:vp}. \red{Suppose $\sft{\Kb_i\pb_R}_{\alpha_i}\rightarrow 1$}, i.e., the tokens $(\alpha_i)_{i=1}^n$ are asymptotically selected. Let $\vs$ be the solution of \eqref{svm-label2} with $\rb_i=\x_{i\alpha_i}$ and $\Nc$ be its set of non-support indices. Suppose Assumption \ref{label margin ass} holds over the support vectors $[n]-\Nc$. Then, $\frac{\vb_r}{r}\rightarrow \frac{\vs}{\tn{\vs}}$ and $\frac{\pb_R}{R}\rightarrow\frac{\prr}{\tn{\prr}}$ where $\prr$ is the solution of \eqref{relax svm} with $\alpha_i$ choices.
%\end{theorem}


%is same as \ref{} with $n=3,T=2$. All three inputs share the point $(0,0)$ which corresponds to their non-optimal tokens. The optimal tokens (denoted by $\star$) are all support vectors of the \eqref{svm-label2} since $\vs=[0,1]$ is the optimal classifier direction (blue color). Because of this, $\ps$ will separate optimal tokens from $(0,0)$ coordinate via \eqref{attnsvm} which results in the red direction (yellow and teal $\star$ are the support tokens).

\begin{comment}
%under generic conditions, 
The following theorem shows that, if the label-margin induced by the first tokens $(\x_{i1})_{i=1}^n$ of each input is larger than the norm of the other tokens, then, mixing the other tokens strictly shrink the label-margin. Consequently, the first tokens naturally become the relevant set and all other tokens become irrelevant.
\begin{theorem} \red{[TO BE PROVEN]} Consider an SVM problem over the dataset $(Y_i,\rb_i)_{i=1}^n$

Suppose all inputs $\rb_i$ are support vectors (all constraints are tight!) and set the margin $\Gamma=1/\tn{\vs}$. Pick points $(\z_i)_{i=1}^n$ and $0\leq \alpha_i\leq 1$ with $\bar{\Gamma}=\sup_{i\in[n]}\tn{\z_i}<\Gamma$. Set $\rb'_i=(1-\alpha_i)\rb_i+\alpha_i\z_i$. Solving SVM over $(Y_i,\rb'_i)$ will lead to a margin of at most $\Gamma-\nu \max_{i\in[n]}\alpha_i$ for some $\nu>0$ (depending on $\Gamma-\bar{\Gamma}$).
\end{theorem}

Note that, the dataset described in this theorem is a generalization of Example \ref{dominant first}. For Example \ref{dominant first}, relevant tokens are simply $\rb_i=\pm \vstar$ and the SVM solution is $\vb^\svm=\vstar/\tn{\vstar}^2$.

\noindent\red{[This seems easy to prove if we just ask $\bar{\Gamma}<\eps\Gamma$ for some small $\eps>0$ (e.g.~by using perturbation argument around $\vs$)]}


. Suppose the problem is separable in the sense that, there are directions

Suppose the regularization path converges to directions $\vs$ and $\ps$. Suppose $\ps$ selects tokens $\bal=(\alpha_i)_{i=1}^n$ from each input $\X_i$. Then, $\vs$ solves \eqref{svm-label2} with $\rb_i=\x_{i\alpha_i}$. Let $\Nc\in[n]$ be the support vectors of $\vs$ solution. Then, $\ps$ is given by the following program
\[
\ps=\arg\min_{\pb}\tn{\pb}\quad\text{subject to}\quad \pb^\top(\kb_{i\alpha_i}-\kb_{it})\geq \begin{cases}1\quad \text{if}\quad i\in \Nc\\0\quad \text{else}\end{cases}.
\]
\smallskip\smallskip\smallskip
\end{comment}

==> sec/bc/joint_05_27.tex <==
%\input{sec/joint_fig.tex}
\section{Joint Convergence of Head $\vba$ and Attention Weights $\pba$}\label{sec joint}\vspace{-5pt}
%\textbf{Joint $\vb,\pb$ convergence:} 


In this section, we extend the preceding results to the general case of joint optimization of head $\vb$ and attention weights $\pb$ using a logistic loss function. To this aim, we focus on regularization path analysis, which involves solving \eqref{lin det losss} under ridge constraints and examining the solution trajectory as the constraints are relaxed. 

\noindent\textbf{High-level intuition.} Since the prediction is linear as a function of $\vb$, logistic regression in $\vb$ can exhibit its own implicit bias to a max-margin solution. Concretely, define the attention features $\x_i^\pb=\X_i^\top\sft{\Kb_i\pb}$ and define the dataset $\Sc^{\pb}=(Y_i,\x_i^\pb)$. If the dataset $\Sc^{\pb}$ is separable by $\vb$, then optimizing only $\vb$ will converge in the direction of the max-margin classifier by setting $\rb_i\gets \x^\pb_i$:
\begin{align}
\vs=\arg\min_{\vb\in\R^d}\tn{\vb}\quad\text{subject to}\quad Y_i\cdot\vb^\top\rb_i\geq 1.\label{svm-label2}\tag{CLS-SVM}
\end{align}
This motivates a clear question:\smallskip
\\\smallskip
\emph{Under what conditions, optimizing $\vb,\pb$ jointly will converge to their respective max-margin solutions?} 
\\
Assuming the dataset is separable by some $(\vb,\pb)$ pair, we start by introducing the optimal token definition for joint convergence. %Assuming that the joint problem is separable and there exists $(\vb,\pb)$ asymptotically achieving zero training loss. 

\noindent\textbf{Optimal tokens} $\op=(\op_i)_{i=1}^n$ are defined to be the selection that maximizes the \eqref{svm-label2} margin subject to being feasible for selection i.e.~$\tn{\ps}<\infty$. Concretely, denote $\vs(\bal)$ to be the solution of \eqref{svm-label2} with $\rb_i\gets \x_{i\alpha_i}$. Then,
\[
\op=\arg\min_{\bal=(\alpha_i)_{i=1}^n} \tn{\vs(\bal)}\quad\text{subject to}\quad \tn{\ps(\bal)}<\infty.
\]
For cleaner notation, we will use $\x^\op_i$ rather than $\x_{i\op_i}$.

We study this question in two steps. Loosely speaking, we will first assume that when solving \eqref{svm-label2}, all inputs $i\in[n]$ are also the support vectors. We will then relax this condition to uncover a more general implicit bias for $\pb$. Throughout we assume that the joint problem is separable and there exists $(\vb,\pb)$ asymptotically achieving zero training loss. %To proceed, we introduce optimal token definition for joint convergence.


%
%The first stage assumes that  where the first phase provides the intuitive answer and second phase establishes a more refine.

%Let us denote the mixed tokens by $\x_i^\pb=\X_i^\top\sft{\Kb_i\pb}$. Given these, we can train a linear classifier $\vb$. Since gradient-descent on logistic regression is biased towards SVM, we introduce the following problem

%Above, we will refer to $1/\tn{\vb^\svm}$ as the \emph{label margin} to distinguish it from attention's \emph{context margin}. 
\vspace{-5pt}
\subsection{When all attention features are support vectors}\vspace{-3pt}
%We will explore the joint implicit bias of $(\vb,\pb)$ when both contexts and labels are separable and optimizing $(\vb,\pb)$ can make logistic loss arbitrarily small. Here,
%To keep notation concise, we assume first token of each input is the optimal choice. The assumption below formalizes this: We assume that, without losing generality,

%The choice of first tokens is for notational convenience and without losing generality. 
Our first insight in quantifying joint implicit bias is that, optimal tokens admit a natural definition: Those that maximize the downstream label margin when selected. This is formalized below where we assume that: (1) selecting the token indices $\bal=(\alpha_i)_{i=1}^n$ from each input data achieves the largest label margin. (2) The optimality of the $\bal$ choice is strict in the sense that mixing other tokens will shrink the label margin in \eqref{svm-label2}. In \eqref{svm-label2}, define \emph{label margin} to be $1/\tn{\vb^\svm}$. 
%assumption in quantifying joint implicit bias is that, if $(\x_i^\pb)_{i=1}^n$ contain irrelevant tokens, then, the label margin of \eqref{svm-label2} strictly shrinks. 
\begin{assumption} \label{label margin ass} Let $\Gamma>0$ be the label margin when solving \eqref{svm-label2} with $\rb_i\gets \x_{i\alpha_i}$. There exists $\nu>0$ such that for all $\pb$, solving \eqref{svm-label2} with $\rb_i\gets \x_i^\pb$ results in a label margin of at most $\Gamma-\nu\cdot \max_{i\in[n]} (1-\s_{i\alpha_i})$ where $\s_i=\sft{\Kb_i\pb}$. 
\end{assumption}
%\begin{assumption} \label{label margin ass} Let $\Gamma>0$ be the label margin when solving \eqref{svm-label2} with $\rb_i\gets \x_{i\alpha_i}$. There exists $\nu>0$ such that for all $\pb$, solving \eqref{svm-label2} with $\rb_i\gets \x_i^\pb$ results in a label margin of at most $\Gamma-\nu\cdot \max_{i\in[n]} (1-\s_{i\alpha_i})$ where $\s_i=\sft{\Kb_i\pb}$. \end{assumption}

%\SO{Is above margin-shrinkage assumption implied by the statement: $\Gamma$ is the unique maximum achievable margin over all $\pb$ (and associated $\rb_i\gets\x_i^\pb$) choices. Essentially, how will the margin shrink in terms of $\max_{i\in[n]}(1-\s_{i\alpha_i})$?}
%\red{\begin{assumption} \label{margin ass better} Let $\Gamma>0$ be the label margin when solving \eqref{svm-label2} with $\rb_i\gets \x_{i\alpha_i}$. $\Gamma$ is the unique maximum margin over all $\pb$ (and associated $\s_i=\sft{\Kb_i\pb}$) choices.\end{assumption}}
%There exists $\nu>0$ such that for all $\pb$, solving \eqref{svm-label2} with $\rb_i\gets \x_i^\pb$ results in a label margin of at most $\Gamma-\nu\cdot \max_{i\in[n]} (1-\s_{i\alpha_i})$ where $\s_i=\sft{\Kb_i\pb}$. 
%A dataset that obeys Theorem \ref{lin det thm} is as follows when we set $\vb=\vstar$. 
%Note that, our choice of first tokens is for notational convenience and without losing generality. 
\noindent\textbf{Example:} To gain intuition, let us fix $\vstar\in\R^d$ and consider the dataset obeying $\x_{i1}=Y_i\cdot \vstar$ and $\tn{\x_{it}}<\tn{\vstar}$ for all $t\geq 2$ and all $i\in[n]$. For this dataset, we can choose $\alpha_i=1$, $\Gamma=\tn{\vstar}$ and $\nu=\tn{\vstar}-\sup_{i\in[n],t\geq 2}\tn{\x_{it}}$.
% maximize downstream margin

\begin{theorem}\label{thm:path:joint:vp} Consider the ridge-constrained solutions $(\vb_r,\pb_R)$ of \eqref{lin det losss} defined as
\[
\vb_r,\pb_R=\underset{\tn{\vb}\leq r,\tn{\pb}\leq R}{\arg\min}\Lc(\vb,\pb).
\]
Suppose Assumption \ref{label margin ass} holds for some $\Gamma,\nu>0$. As $r,R\rightarrow\infty$, the joint regularization path $(\vb_r,\pb_R)$ converges as follows:
\begin{itemize}
\item   $\frac{\pb_R}{R}\rightarrow\frac{\ps}{\tn{\ps}}$ where $\ps$ is the solution of \eqref{attnsvm}; and
\item $\frac{\vb_{r}}{r}\rightarrow \frac{\vs}{\tn{\vs}}$ where $\vs$ is the solution of \eqref{svm-label2} with $\rb_i=\x_{i1}$.
\end{itemize}
\end{theorem}

As further discussion, consider Figure \ref{fig2:allsvm} where we set $n=3,T=d=2$ and $\W=\text{Identity}$. All three inputs share the point $(0,0)$ which corresponds to their non-optimal tokens. The optimal tokens (denoted by $\star$) are all support vectors of the \eqref{svm-label2} since $\vs=[0,1]$ is the optimal classifier direction (blue color). Because of this, $\ps$ will separate optimal tokens from $(0,0)$ coordinate via \eqref{attnsvm} which results in the red direction (yellow and teal $\star$ are the support tokens).
%Set $\bar{\Gamma}=\sup_{t\neq \alpha_i} \tn{\x_{ti}}<\Gamma$. 

\input{sec/joint_fig.tex}
\vspace{-5pt}
\subsection{General solution when selecting one token per input}\vspace{-3pt}

%, and without losing generality, again assume $\alpha_i=1$
Can we relax Assumption \ref{label margin ass}, and if so, what is the resulting behavior? Consider the scenario where the optimal $\pb$ diverges to $\infty$ and ends up selecting one token per input. Suppose this $\pb$ selects some coordinates $\bal=(\alpha_i)_{i=1}^n$. Let $\Nc\subset[n]$ be the set of indices where the associated token $\x_{i\alpha_i}$ is \textbf{not} a support vector when solving \eqref{svm-label2}. Our intuition is as follows: Even if we slightly perturb this $\pb$ choice and mix other tokens $t\neq \alpha_i$ over the input set $\Nc\subset[n]$, since $\Nc$ is not support vector for \eqref{svm-label2}, we can preserve the label margin (by only preserving the support vectors $[n]-\Nc$). This means that $\pb$ may not have to enforce \emph{max-margin} constraint over inputs $i\in\Nc$, instead, it suffices to just select these tokens (asymptotically). This results in the following \textbf{relaxed SVM} problem:
\begin{align} 
\prr=\min_{\pb} \tn{\pb}\quad\text{such that}\quad \pb^\top (\kb_{i\alpha_i}-\kb_{it})\geq \begin{cases} 1\quad\text{for all}\quad t\neq \alpha_i,~i\in[n]-\Nc\\ 0\quad\text{for all}\quad t\neq \alpha_i,~i\in\Nc\end{cases}.\label{relax svm}
\end{align}
Here, $\pb^\top \x_{i\alpha_i}\geq 0$ corresponds to the \emph{selection} idea. Building on this intuition, the following theorem captures the generalized behavior of the joint regularization path.
%for some indices $(\alpha_i)_{i=1}^n$, 
%$\x^{\pb_R}_i:=\X_i^\top\sft{\Kb_i\pb_R}\rightarrow \x_{i\alpha_i}$
%Let $\eb_j$ be the $j$'th standard basis vector. 
%\begin{theorem}\label{joint thm general} Consider the path of $(\vb_r,\pb_R)$ as $r,R\rightarrow\infty$ as in Theorem \ref{thm:path:joint:vp}. \red{Suppose $\sft{\Kb_i\pb_R}_{\alpha_i}\rightarrow 1$}, i.e., the tokens $(\alpha_i)_{i=1}^n$ are asymptotically selected. Then, $\vb_{r}/{r}\rightarrow \vs/\tn{\vs}$ where $\vs$ is the solution of \eqref{svm-label2} with $\rb_i=\x_{i\alpha_i}$, $\Nc$ is the set of non-support vectors for \eqref{svm-label2}, and $\frac{\pb_R}{R}\rightarrow\frac{\prr}{\tn{\prr}}$ where $\prr$ is the solution of \eqref{relax svm} with $\alpha_i$ choices.
%\end{theorem}
%\SO{Does $\sft{\Kb_i\pb_R}_{\alpha_i}\rightarrow 1$ above imply margin-shrinkage Assumption \ref{label margin ass} when we mix non-$\alpha_i$ tokens (over support vectors)? Otherwise, we need to add the sentence ``Suppose Assumption \ref{label margin ass} holds over the support vectors $[n]-\Nc$.''}
\begin{theorem}\label{joint thm general} Consider the path of $(\vb_r,\pb_R)$ as $r,R\rightarrow\infty$ as in Theorem \ref{thm:path:joint:vp}. {Suppose $\sft{\Kb_i\pb_R}_{\alpha_i}\rightarrow 1$}, i.e., the tokens $(\alpha_i)_{i=1}^n$ are asymptotically selected. Let $\vs$ be the solution of \eqref{svm-label2} with $\rb_i=\x_{i\alpha_i}$ and $\Nc$ be its set of non-support indices. Suppose Assumption \ref{label margin ass} holds over the support vectors $[n]-\Nc$. Then, $\frac{\vb_r}{r}\rightarrow \frac{\vs}{\tn{\vs}}$ and $\frac{\pb_R}{R}\rightarrow\frac{\prr}{\tn{\prr}}$ where $\prr$ is the solution of \eqref{relax svm} with $\alpha_i$ choices.
\end{theorem}
To illustrate this numerically, consider Figure \ref{fig2:nosvm} which modifies Figure \ref{fig2:allsvm} by pushing the yellow $\star$ to the northern position $(0.5,1.5)$. We still have $\vs=[0,1]$ however the yellow $\star$ is no longer a support vector of \eqref{svm-label2}. Thus, $\pb$ solves the relaxed problem which separates green and teal $\star$'s by enforcing the max-margin constraint on $\pb$ (which is the red direction). Instead, yellow $\star$ only needs to achieve positive correlation with $\pb$ (unlike Figure \ref{fig2:allsvm} where it dictates the direction).




%is same as \ref{} with $n=3,T=2$. All three inputs share the point $(0,0)$ which corresponds to their non-optimal tokens. The optimal tokens (denoted by $\star$) are all support vectors of the \eqref{svm-label2} since $\vs=[0,1]$ is the optimal classifier direction (blue color). Because of this, $\ps$ will separate optimal tokens from $(0,0)$ coordinate via \eqref{attnsvm} which results in the red direction (yellow and teal $\star$ are the support tokens).

\begin{comment}
%under generic conditions, 
The following theorem shows that, if the label-margin induced by the first tokens $(\x_{i1})_{i=1}^n$ of each input is larger than the norm of the other tokens, then, mixing the other tokens strictly shrink the label-margin. Consequently, the first tokens naturally become the relevant set and all other tokens become irrelevant.
\begin{theorem} \red{[TO BE PROVEN]} Consider an SVM problem over the dataset $(Y_i,\rb_i)_{i=1}^n$. Suppose all inputs $\rb_i$ are support vectors (all constraints are tight!) and set the margin $\Gamma=1/\tn{\vs}$. Pick points $(\z_i)_{i=1}^n$ and $0\leq \alpha_i\leq 1$ with $\bar{\Gamma}=\sup_{i\in[n]}\tn{\z_i}<\Gamma$. Set $\rb'_i=(1-\alpha_i)\rb_i+\alpha_i\z_i$. Solving SVM over $(Y_i,\rb'_i)$ will lead to a margin of at most $\Gamma-\nu \max_{i\in[n]}\alpha_i$ for some $\nu>0$ (depending on $\Gamma-\bar{\Gamma}$).
\end{theorem}

Note that, the dataset described in this theorem is a generalization of Example \ref{dominant first}. For Example \ref{dominant first}, relevant tokens are simply $\rb_i=\pm \vstar$ and the SVM solution is $\vb^\svm=\vstar/\tn{\vstar}^2$.

\noindent\red{[This seems easy to prove if we just ask $\bar{\Gamma}<\eps\Gamma$ for some small $\eps>0$ (e.g.~by using perturbation argument around $\vs$)]}


. Suppose the problem is separable in the sense that, there are directions

Suppose the regularization path converges to directions $\vs$ and $\ps$. Suppose $\ps$ selects tokens $\bal=(\alpha_i)_{i=1}^n$ from each input $\X_i$. Then, $\vs$ solves \eqref{svm-label2} with $\rb_i=\x_{i\alpha_i}$. Let $\Nc\in[n]$ be the support vectors of $\vs$ solution. Then, $\ps$ is given by the following program
\[
\ps=\arg\min_{\pb}\tn{\pb}\quad\text{subject to}\quad \pb^\top(\kb_{i\alpha_i}-\kb_{it})\geq \begin{cases}1\quad \text{if}\quad i\in \Nc\\0\quad \text{else}\end{cases}.
\]
\smallskip\smallskip\smallskip
\end{comment}

==> sec/bc/meta_thm_04_02.tex <==
\section{A Generic Result on the Regularization Path of Attention}

%Our results will build on a contextual dataset model where the high-level idea is splitting a tokenized input into label-relevant and label-irrelevant tokens\footnote{In Section \ref{multicon}, we also augment this model to allow for multiple contexts akin to the distinction between binary vs multiclass classification.}. Under this model, we will see that attention mechanism plays a critical for separating relevant tokens from the irrelevant ones.

The goal of this section is identifying generic conditions that lead to the implicit bias of softmax-attention. Thus, we will first state a meta-theorem that works under minimal assumptions on the dataset. Later sections identify additional assumptions to obtain additional/stronger results.
%\noindent\textbf{Training Dataset:} 
Let $\Sc=(\X_i,Y_i)_{i=1}^n$ be a dataset of input-label pairs where $Y_i\in\R$ is the label and $\X_i\in\R^{T\times d}$ is the tokenized input features. The high-level intuition is that, in order for softmax-attention to exhibit optimization bias, the optimization problem should be forced to separate relevant tokens from irrelevant ones. We shall formalize this idea for the nonlinear model \eqref{npatt}. Let $\ell(Y,\hat{Y})$ be a loss function and consider the training risk
\begin{align}
\Lc(\pb)=\frac{1}{n}\sum_{i=1}^n \ell(Y_i,\link{\X_i^\top \ab_i})\quad\text{where}\quad\ab_i=\sft{\Kb_i\pb}\in\R^T.\label{NPT loss}
\end{align}
Above, $\Kb_i:=\W^\top\X_i$ is the key features following \eqref{patt}. Our theory will build on a contextual data assumption where the high-level idea is splitting tokens of the input $\X_i$ into a label-relevant set $\Rc_i\in [T]$ and label-irrelevant set $\Rcb_i=[T]-\Rc_i$. The key question is how to define the notion of \emph{relevant set}. The assumption below introduces a generic definition where irrelevant tokens are those that strictly increase the training risk $\Lc(\pb)$ if they are not fully suppressed by softmax-attention output $\ab_i$. Below $a\wedge b$ denotes the minimum of two scalars $a$ and $b$.
% and label-irrelevant tokenshigh-level intuition the $T$ tokens of each input $\X_i$ into a label-relevant set  

%Above, attention weights $\ab_i$ are calculated with $\Cb_i$ which is the context matrix obtained by filtering value information from $\X_i$. This is helpful to obtain a clean context separation result for the nonlinear $\lnk$ setting. Under linear value Assumption \ref{linass}, we also develop results for the standard model $\ab_i=\sft{\Cb_i\qb}$.  
%\hat{\qb}_R=\arg\min_{\tn{\qb}\leq R}\Lc(\qb)\quad\text{where}\quad 
%Denote $\Lc_\st=\min_{\pb}\Lc(\pb)$. 
\begin{assumption} [Mixing irrelevant tokens hurt]\label{asshurt} Let $s^{\pb}_i=\sum_{t\in \Rcb_{i}} \ab_{it}$ be the sum of softmax similarities over the irrelevant set for $\pb$. Let $s^{\pb}_{\max}=\max_{i \in [n]}s^{\pb}_i$ be the worst-case irrelevance. For any $\Delta>0$, there exists $\rho<0$ such that for all $\pb,\pb'$ obeying
\[
\log (s^{\pb}_{\max})\leq (1+\Delta)\log (s^{\pb'}_{\max})\wedge \rho,
\]
we have that $\Lc(\pb)< \Lc(\pb')$.
\end{assumption}
Above, we say \emph{mixing hurts} because $\X_i^\top \ab_i$ is mixing the tokens of $\X_i$ and our condition is that, to achieve optimal risk, this mixture should not contain any irrelevant tokens. More specifically, we require that, a model $\pb$ that contain \emph{exponentially less irrelevance} (quantified via log-$s_{\max}$) compared to $\pb'$ is strictly preferable. See Section \ref{sec:linear data} below for a concrete problem instance with a linear classifier head satisfying this condition.

Finally, before stating our generic theorem, we need to introduce the max-margin separator towards which attention is implicitly biased. This is given by the solution to the following SVM-type optimization problem that separates relevant and irrelevant tokens
\begin{align}
    \pb^{\svm}=\arg\min_{\pb}\tn{\pb}\quad\text{subject to}\quad &m_i\geq 1\quad\text{for all}\quad i\in [n]\label{svm}\tag{SVM}\\
    \text{where}\quad &m_i:=\max_{\alpha\in \Rc_{i}}\min_{\beta\in \Rcb_{i}}\pb^\top(\kb_{i\alpha}-\kb_{i\beta}).\nn
\end{align}
\noindent\textbf{Remark:} We note that this problem is not convex as $m_i\geq 1$ constraint can be nonconvex when relevant set $\Rc_i$ is not a singleton. To see this, imagine $n=d=1$ and $T=3$: Set two relevant tokens as $\kb_1=1$ and $\kb_2=-1$ and the irrelevant token as $\kb_3=0$. The optimal solutions of \eqref{svm} are $\pb^\svm=\pm 1$. On the other hand, problem becomes convex if there is a single relevant token or all relevant tokens are identical so that application of $\max_{\alpha\in \Rc_{i}}$ becomes trivial.

\noindent\textbf{Interpretation:} Each input $\X_i$ has an associated key matrix $\Kb$ with $T$ tokens $(\kb_{it})_{t=1}^T$. We aim to achieve the maximum margin $m_i$ in order to separate the single best relevant token from all irrelevant tokens. Additionally, we wish to accomplish this goal for all inputs in the dataset, thus, we need to find the best $\pb$ that ensures all margins obey $m_i\geq 1$.

\begin{theorem} Suppose Assumption \ref{asshurt} holds. Let $\Pc^\svm$ be the set of global minima of \eqref{svm}. Suppose the cost $\Gamma:=\tn{\pb^\svm}$ is finite. Define the regularization path of \eqref{NPT loss} as $\pb_R=\arg\min_{\tn{\pb}\leq R}\Lc(\pb)$. Then, we have that
\[
\lim_{R\to\infty}\dist{\Gamma\frac{\pb_R}{R},\Pc^\svm}=0.
\]
Here $\dist{\cdot,\cdot}$ denotes the Euclidean distance of a vector to a set.
\end{theorem}
In words, this theorem shows that, as the regularization strength $R$ is relaxed to obtain the ridgeless optimization $\min_{\pb}\Lc(\pb)$, the direction of the optimal $\pb_R$ converges to a max-margin separator $\pb^{\svm}\in \Pc^\svm$ of \eqref{max-margin}. 

\begin{proof} The key idea is showing that, thanks to the exponential tail of softmax-attention, (harmful) contribution of the irrelevant token with the minimum margin can dominate the contribution of all other tokens as $R\rightarrow\infty$. This high-level approach is similar to earlier works on implicit bias of gradient descent with logistic loss.

Pick $\pb^\svm\in \Pc^\svm$ and set $\pb^\st_R=R\frac{\pb^\svm}{\tn{\pb^\svm}}$. This will be the baseline model that $\pb_R$ has to compete against. Also let $\pbb_R=\Gamma\frac{\pb_R}{R}$. Now suppose $\dist{\pbb_R, \Pc^\svm}\not\rightarrow0$ as $R\rightarrow\infty$. Then, there exists $\delta>0$ such that, we can always find arbitrarily large $R$ obeying $\dist{\pbb_R, \Pc^\svm}\geq \delta$.

Since $\pbb_R$ is $\delta>0$ bounded away from $\Pc^\svm$, $\pbb_R$ and $\tn{\pbb_R}=\tn{\pb^\svm}$, $\pbb_R$ strictly violates at least one of the inequality constraints in \eqref{svm}. Otherwise, we would have $\pbb_R\in \Pc^\svm$. Without losing generality, suppose $\pbb_R$ violates the constraint $m_1\geq 1$, that is, for some $\gamma:=\gamma(\delta)>0$, $\max_{t_1\in \Rc_{i}}\min_{t_0\in \Rcb_{i}}\pb^\top(\kb_{it_1}-\kb_{it_0})\leq 1-\gamma$. Now, we will argue that this will lead to a contradiction as $R\rightarrow\infty$ since we will show that $\Lc(\pb^\st_R)<\Lc(\pb_R)$ for sufficiently large $R$.

First, let us control $\Lc(\pb^\st_R)$. We study $\ab^\st_i=\sft{\Kb_i\pb^\st_R}$ and let $\alpha_i\in\Rc_i$ be the index $\alpha$ in \eqref{svm} for which $m_i\geq 1$ is attained. Then, we bound the irrelevant $s^\st_i$ of $\pb^\st_R$ as
\[
s^\st_i=\frac{\sum_{t\in \Rcb_{i}}\exp(\kb_{it}^\top \pb^\st_R)}{\sum_{t\in [T]}\exp(\kb_{it}^\top \pb^\st_R)}\leq \frac{\sum_{t\in \Rcb_{i}}\exp(\kb_{it}^\top \pb^\st_R)}{\exp(\kb_{i\alpha_i}^\top \pb^\st_R)}\leq T\exp(-R/\Gamma).
\]
Thus, $s^\st_{\max}=\max_{i\in [n]}s^\st_i\leq T\exp(-R/\Gamma)$. Secondly, we wish to control $\Lc(\pb_R)$ by lower bounding the irrelevance in $\pb_R$. Focusing on $m_1$, let $\alpha\in\Rc_1$ be the index in \eqref{svm} for which $m_1\leq 1-\gamma$ is attained. Denoting irrelevant weight-sum in the first input as $\hat{s}_1$, we find
\[
\hat{s}_1=\frac{\sum_{t\in \Rcb_{1}}\exp(\kb_{1t}^\top \pb_R)}{\sum_{t\in [T]}\exp(\kb_{1t}^\top \pb_R)}\geq \frac{1}{T}\frac{\sum_{t\in \Rcb_{1}}\exp(\kb_{1t}^\top \pb_R)}{\exp(\kb_{1\alpha}^\top \pb_R)}\geq T^{-1}\exp(-R(1-\gamma)/\Gamma).
\]
We similarly have $s^\st_{\max}\geq T^{-1}\exp(-R\Gamma)$. In conclusion, for $\pb_R,\pb^\st_R$, denoting maximum irrelevances by $\hat{s}_{\max}\geq \hat{s}_1$ and $s^\st_{\max}$, we respectively obtained 
\begin{align*}
\log(\hat{s}_{\max})&\geq -(1-\gamma)(R/\Gamma)-\log T,\\
 -(R/\Gamma)-\log T\leq \log(s^\st_{\max})&\leq -(R/\Gamma)+\log T.
\end{align*}
The above inequalities satisfy Assumption \ref{asshurt} as follows where $\pb\gets\pb^\star_R$ and $\pb'\gets \pb_R$: Set $R_0=3\gamma^{-1}\Gamma\log T$ so that $\log T\leq \frac{\gamma R_0}{3\Gamma}$. Secondly, set $\rho_0=-(R_0/\Gamma)-\log T$. This way, $\rho_0\geq \log(s^\st_{\max})$ implies $R\geq R_0$ and $\log T\leq \frac{\gamma R}{3\Gamma}$. To proceed, using the latter inequality, we bound the $\log T$ terms to obtain
\begin{itemize}
\item $\log(\hat{s}_{\max})\geq -(1-2\gamma/3)(R/\Gamma)$.
\item $\log(s^\st_{\max})\leq -(1-\gamma/3)(R/\Gamma)$.
\end{itemize}
To proceed, we pick $1+\Delta=\frac{1-\gamma/3}{1-2\gamma/3}$ implying $\Delta:=\frac{\gamma}{3-2\gamma}$. Finally, for this $\Delta$, there exists $\rho(\Delta)$ which we need to ensure $\log(\hat{s}_{\max})\leq \rho(\Delta)$. This can be guaranteed by picking sufficiently large $R$ that ensures $\log(s^\st_{\max})\leq -(1-\gamma/3)(R/\Gamma)\leq \rho(\Delta)$ to satisfy all conditions of Assumption \ref{asshurt}. Since such large $R$ exists by initial assumption $\dist{\pbb_R, \Pc^\svm}\not\rightarrow0$, Assumption \ref{asshurt} in turn implies that $\Lc(\pb^\st_R)<\Lc(\pb_R)$ contradicting with the optimality of $\pb_R$ in \eqref{NPT loss}.
\end{proof}
% for sufficiently small $$ $R\geq R_0$ (which exists by initial assumption)
The following example will be further elaborated in Section \ref{sec:linear data} and shows that if irrelevant tokens result in label noise, Assumption \ref{asshurt} holds.%and $s_{\max}^{\pb}=\max_{i\in[n]}s^{\pb}_i$ 
\begin{lemma} [Linear label mixing] Recall $s^{\pb}_i=\sum_{t\in \Rcb_t}\ab_{it}$ from Assumption \ref{asshurt}. Suppose $\link{\X_i^\top \ab_i}=\nu(1-s_i^{\pb})Y_i+Z_i$ for some $\nu> 0$. Here $Z_i$ is a zero-mean label-noise variable induced by the irrelevant tokens. For some $C>0$, $\E[Z_i^2]^{1/2}\leq Cs^{\pb}_{\max}$ for all $\pb$ (allowing for $Z_i=0$). Consider the expected loss over $Z_i$, namely, $\bar{\Lc}(\pb):=\E_{(Z_i)_{i=1}^n}[\Lc(\pb)]$. Then, Assumption \ref{asshurt} holds for $\bar{\Lc}(\pb)$ when either of the following conditions hold:
    \begin{itemize} 
        \item Suppose $\ell(\cdot)$ is the quadratic loss, labels $Y_i$ are arbitrary but nonzero, and $\nu\leq 1$.
        \item Suppose $\ell(\cdot)$ is the logistic loss, labels $Y_i\in\{-1,1\}$, and $\nu$ is arbitrary.
    \end{itemize}
\end{lemma}
\begin{proof} \noindent\textbf{$\bullet$ Case 1: Quadratic loss.} Let us first consider the quadratic loss. Denote $\sigma_i^2=\E[Z_i^2]\leq s_{\max}^2$ and let $M_+=\max_{i\in[n]}Y_i^2,M_-=\min_{i\in[n]}Y_i^2>0$. We have that
    %$\sigma_{\max}^2=\max_{i\in[n]}\sigma_i^2$
    \begin{align}
    \bar{\Lc}(\pb)&=\frac{1}{n}\sum_{i=1}^n\E_{Z_i}[(Y_i-\nu (1-s_i)Y_i-Z_i)^2]= \frac{1}{n}\sum_{i=1}^n((1-\nu+\nu s_i)^2Y_i^2+\sigma_i^2)\\
    &\geq B:=(1-\nu+\nu s_{\max})^2M_-/n.
    \end{align}
    Using same argument and upper bound on $\E[Z_i^2]$, we also obtain an upper bound
    \[
    \bar{\Lc}(\pb)\leq (1-\nu+\nu s_{\max})^2M_++C^2s_{\max}^2.
    \]
    Now, independent of the choice of $\pb$, the ratio of upper/lower bounds obey (using $s_{\max}\leq 1$) 
    \[
    \frac{(1-\nu+\nu s_{\max})^2M_++C^2s_{\max}^2}{B:=(1-\nu+\nu s_{\max})^2M_-/n}\leq n\frac{M_++C^2}{M_-}:=\Theta.
    \] 
    %Recalling $s_{\max}:=\max_{i\in[n]}s_i$, clearly,
    %Setting $B:=(1-\nu+\nu s_{\max})\sqrt{M_-/n}$, 
    Overall, we found $\sqrt{\Theta}B\geq \sqrt{\bar{\Lc}(\pb)}\geq B$. Thus, for any $\pb,\pb'$, we have that, if $\sqrt{\Theta } (1-\nu+\nu s_{\max}^{\pb})< (1-\nu+\nu s_{\max}^{\pb'})$, then $\Lc(\pb)< \Lc(\pb')$. Note that this condition is implied by the stricter criteria $\sqrt{\Theta } s_{\max}^{\pb}< s_{\max}^{\pb'}$.
    
    Going back to Assumption \ref{asshurt}, any $\log (s^{\pb}_{\max})\leq (1+\Delta)\log (s^{\pb'}_{\max})$ obeys $s^{\pb}_{\max}\leq (s^{\pb'}_{\max})^{1+\Delta}$ i.e. $s^{\pb'}_{\max}\geq (s^{\pb}_{\max})^{(1+\Delta)^{-1}}$. We wish to ensure $s^{\pb'}_{\max}>\sqrt{n}s^{\pb}_{\max}$, which is guaranteed by
    \[
    (s^{\pb}_{\max})^{(1+\Delta)^{-1}-1}>\sqrt{n}\iff \frac{\Delta}{1+\Delta}\log(s^{\pb}_{\max})< -0.5\log(n),
    \]
    satisfied by choosing a $\rho(\Delta)< -(1+\Delta^{-1})\log(n)$.

    \noindent\textbf{$\bullet$ Case 2: Logistic loss.} Logistic loss is relevant because (i) it is used in most classification problems and also (ii) softmax-attention and logistic loss are both exponential-tailed so their joint interaction is of practical interest for transformers. To proceed, let us write the logistic loss in a similar fashion where we use $\ell(Y,\hat{Y})=-\log(Y\hat{Y})$. Note that $Z'_i=Y_iZ_i\sim Z_i$.
    \begin{align*}
    \bar{\Lc}(\pb)&=\frac{1}{n}\sum_{i=1}^n\E_{Z_i}[-\log(Y_i((1-s_i^{\pb})Y_i+s_i^{\pb} Z_i))]\\
    &=\frac{1}{n}\sum_{i=1}^n\E_{Z_i}[-\log((1-s_i^{\pb})+s_i^{\pb} Z'_i)]\\
    &=\frac{-1}{2n}\sum_{i=1}^n[\log((1-s_i^{\pb})+s_i^{\pb} \eps)+\log((1-s_i^{\pb})-s_i^{\pb} \eps)]\\
    &=\frac{-1}{2n}\sum_{i=1}^n\log((1-s_i^{\pb})^2-\eps^2s_i^{\pb})
    \end{align*}
\end{proof}
%Let $\x_{i\alpha},\x_{i\beta}$ be arbitrary relevant and irrelevant tokens in $\X_i$ respectively. Suppose $\link{\x_{i\alpha}}=Y_i$ and $\link{\x_{i\beta}}=Z_i$ where $Z_i$ is the label-noise induced by the irrelevant tokens. Suppose $Z_i$ is random and for some $p,\eps>0$ $\P(Z_iY_i<-\eps)>p$. Then, Assumption \ref{asshurt} holds when $\ell$ is quadratic loss or for some there exists 
    %$allowed to be stochastic but there exists $ 
%\ab^\st_{it}
% To see this, consider the following optimization problem
% This implies that there exists $\eps>0$ such that $\tn{\pbb-\pb^\svm}\geq \eps$ for all $R\geq \delta^{-1}$. Now, consider the following optimization problem
    



%\begin{example}\label{linear example}\end{example}

==> sec/bc/meta_thm_04_03.tex <==
\section{A Generic Result on the Regularization Path of Attention}

%Our results will build on a contextual dataset model where the high-level idea is splitting a tokenized input into label-relevant and label-irrelevant tokens\footnote{In Section \ref{multicon}, we also augment this model to allow for multiple contexts akin to the distinction between binary vs multiclass classification.}. Under this model, we will see that attention mechanism plays a critical for separating relevant tokens from the irrelevant ones.

The goal of this section is identifying generic conditions that lead to the implicit bias of softmax-attention. Thus, we will first state a meta-theorem that works under minimal assumptions on the dataset. Later sections identify additional assumptions to obtain additional/stronger results.
%\noindent\textbf{Training Dataset:} 
Let $\Sc=(\X_i,Y_i)_{i=1}^n$ be a dataset of input-label pairs where $Y_i\in\R$ is the label and $\X_i\in\R^{T\times d}$ is the tokenized input features. The high-level intuition is that, in order for softmax-attention to exhibit optimization bias, the optimization problem should be forced to separate relevant tokens from irrelevant ones. We shall formalize this idea for the nonlinear model \eqref{npatt}. Let $\ell(Y,\hat{Y})$ be a loss function and consider the training risk
\begin{align}
\Lc(\pb)=\frac{1}{n}\sum_{i=1}^n \ell(Y_i,\link{\X_i^\top \ab_i})\quad\text{where}\quad\ab_i=\sft{\Kb_i\pb}\in\R^T.\label{NPT loss}
\end{align}
Above, $\Kb_i:=\W^\top\X_i$ is the key features following \eqref{patt}. Our theory will build on a contextual data assumption where the high-level idea is splitting tokens of the input $\X_i$ into a label-relevant set $\Rc_i\in [T]$ and label-irrelevant set $\Rcb_i=[T]-\Rc_i$. The key question is how to define the notion of \emph{relevant set}. The assumption below introduces a generic definition where irrelevant tokens are those that strictly increase the training risk $\Lc(\pb)$ if they are not fully suppressed by softmax-attention output $\ab_i$. Below $a\wedge b$ denotes the minimum of two scalars $a$ and $b$.
% and label-irrelevant tokenshigh-level intuition the $T$ tokens of each input $\X_i$ into a label-relevant set  

%Above, attention weights $\ab_i$ are calculated with $\Cb_i$ which is the context matrix obtained by filtering value information from $\X_i$. This is helpful to obtain a clean context separation result for the nonlinear $\lnk$ setting. Under linear value Assumption \ref{linass}, we also develop results for the standard model $\ab_i=\sft{\Cb_i\qb}$.  
%\hat{\qb}_R=\arg\min_{\tn{\qb}\leq R}\Lc(\qb)\quad\text{where}\quad 
%Denote $\Lc_\st=\min_{\pb}\Lc(\pb)$. 
\begin{assumption} [Mixing irrelevant tokens hurt]\label{asshurt} Let $s^{\pb}_i=\sum_{t\in \Rcb_{i}} \ab_{it}$ be the sum of softmax similarities over the irrelevant set for $\pb$. Let $s^{\pb}_{\max}=\max_{i \in [n]}s^{\pb}_i$ be the worst-case irrelevance. For any $\Delta>0$, there exists $\rho<0$ such that for all $\pb,\pb'$ obeying
\[
\log (s^{\pb}_{\max})\leq (1+\Delta)\log (s^{\pb'}_{\max})\wedge \rho,
\]
we have that $\Lc(\pb)< \Lc(\pb')$.
\end{assumption}
Above, we say \emph{mixing hurts} because $\X_i^\top \ab_i$ is mixing the tokens of $\X_i$ and our condition is that, to achieve optimal risk, this mixture should not contain any irrelevant tokens. More specifically, we require that, a model $\pb$ that contain \emph{exponentially less irrelevance} (quantified via log-$s_{\max}$) compared to $\pb'$ is strictly preferable. See Section \ref{sec:linear data} below for a concrete problem instance with a linear classifier head satisfying this condition.

Finally, before stating our generic theorem, we need to introduce the max-margin separator towards which attention is implicitly biased. This is given by the solution to the following SVM-type optimization problem that separates relevant and irrelevant tokens
\begin{align}
\pb^{\svm}=\arg\min_{\pb}\tn{\pb}\quad\text{subject to}\quad &m_i\geq 1\quad\text{for all}\quad i\in [n]\label{svm}\tag{SVM}\\
\text{where}\quad &m_i:=\max_{\alpha\in \Rc_{i}}\min_{\beta\in \Rcb_{i}}\pb^\top(\kb_{i\alpha}-\kb_{i\beta}).\nn
\end{align}
\noindent\textbf{Remark:} We note that this problem is not convex as $m_i\geq 1$ constraint can be nonconvex when relevant set $\Rc_i$ is not a singleton. To see this, imagine $n=d=1$ and $T=3$: Set two relevant tokens as $\kb_1=1$ and $\kb_2=-1$ and the irrelevant token as $\kb_3=0$. The optimal solutions of \eqref{svm} are $\pb^\svm=\pm 1$. On the other hand, problem becomes convex if there is a single relevant token or all relevant tokens are identical so that application of $\max_{\alpha\in \Rc_{i}}$ becomes trivial.

\noindent\textbf{Interpretation:} Each input $\X_i$ has an associated key matrix $\Kb$ with $T$ tokens $(\kb_{it})_{t=1}^T$. We aim to achieve the maximum margin $m_i$ in order to separate the single best relevant token from all irrelevant tokens. Additionally, we wish to accomplish this goal for all inputs in the dataset, thus, we need to find the best $\pb$ that ensures all margins obey $m_i\geq 1$.

\begin{theorem} \label{meta thm} Suppose Assumption \ref{asshurt} holds. Let $\Pc^\svm$ be the set of global minima of \eqref{svm}. Suppose the cost $\Gamma:=\tn{\pb^\svm}$ is finite. Define the regularization path of \eqref{NPT loss} as $\pb_R=\arg\min_{\tn{\pb}\leq R}\Lc(\pb)$. Then, we have that
\[
\lim_{R\to\infty}\dist{\Gamma\frac{\pb_R}{R},\Pc^\svm}=0.
\]
Here $\dist{\cdot,\cdot}$ denotes the Euclidean distance of a vector to a set.
\end{theorem}
In words, this theorem shows that, as the regularization strength $R$ is relaxed to obtain the ridgeless optimization $\min_{\pb}\Lc(\pb)$, the direction of the optimal $\pb_R$ converges to a max-margin separator $\pb^{\svm}\in \Pc^\svm$ of \eqref{max-margin}. 

\begin{proof} The key idea is showing that, thanks to the exponential tail of softmax-attention, (harmful) contribution of the irrelevant token with the minimum margin can dominate the contribution of all other tokens as $R\rightarrow\infty$. This high-level approach is similar to earlier works on implicit bias of gradient descent with logistic loss.

Pick $\pb^\svm\in \Pc^\svm$ and set $\pb^\st_R=R\frac{\pb^\svm}{\tn{\pb^\svm}}$. This will be the baseline model that $\pb_R$ has to compete against. Also let $\pbb_R=\Gamma\frac{\pb_R}{R}$. Now suppose $\dist{\pbb_R, \Pc^\svm}\not\rightarrow0$ as $R\rightarrow\infty$. Then, there exists $\delta>0$ such that, we can always find arbitrarily large $R$ obeying $\dist{\pbb_R, \Pc^\svm}\geq \delta$.

Since $\pbb_R$ is $\delta>0$ bounded away from $\Pc^\svm$, $\pbb_R$ and $\tn{\pbb_R}=\tn{\pb^\svm}$, $\pbb_R$ strictly violates at least one of the inequality constraints in \eqref{svm}. Otherwise, we would have $\pbb_R\in \Pc^\svm$. Without losing generality, suppose $\pbb_R$ violates the constraint $m_1\geq 1$, that is, for some $\gamma:=\gamma(\delta)>0$, $\max_{t_1\in \Rc_{i}}\min_{t_0\in \Rcb_{i}}\pb^\top(\kb_{it_1}-\kb_{it_0})\leq 1-\gamma$. Now, we will argue that this will lead to a contradiction as $R\rightarrow\infty$ since we will show that $\Lc(\pb^\st_R)<\Lc(\pb_R)$ for sufficiently large $R$.

First, let us control $\Lc(\pb^\st_R)$. We study $\ab^\st_i=\sft{\Kb_i\pb^\st_R}$ and let $\alpha_i\in\Rc_i$ be the index $\alpha$ in \eqref{svm} for which $m_i\geq 1$ is attained. Then, we bound the irrelevant $s^\st_i$ of $\pb^\st_R$ as
\[
s^\st_i=\frac{\sum_{t\in \Rcb_{i}}\exp(\kb_{it}^\top \pb^\st_R)}{\sum_{t\in [T]}\exp(\kb_{it}^\top \pb^\st_R)}\leq \frac{\sum_{t\in \Rcb_{i}}\exp(\kb_{it}^\top \pb^\st_R)}{\exp(\kb_{i\alpha_i}^\top \pb^\st_R)}\leq T\exp(-R/\Gamma).
\]
Thus, $s^\st_{\max}=\max_{i\in [n]}s^\st_i\leq T\exp(-R/\Gamma)$. Secondly, we wish to control $\Lc(\pb_R)$ by lower bounding the irrelevance in $\pb_R$. Focusing on $m_1$, let $\alpha\in\Rc_1$ be the index in \eqref{svm} for which $m_1\leq 1-\gamma$ is attained. Denoting irrelevant weight-sum in the first input as $\hat{s}_1$, we find
\[
\hat{s}_1=\frac{\sum_{t\in \Rcb_{1}}\exp(\kb_{1t}^\top \pb_R)}{\sum_{t\in [T]}\exp(\kb_{1t}^\top \pb_R)}\geq \frac{1}{T}\frac{\sum_{t\in \Rcb_{1}}\exp(\kb_{1t}^\top \pb_R)}{\exp(\kb_{1\alpha}^\top \pb_R)}\geq T^{-1}\exp(-R(1-\gamma)/\Gamma).
\]
We similarly have $s^\st_{\max}\geq T^{-1}\exp(-R\Gamma)$. In conclusion, for $\pb_R,\pb^\st_R$, denoting maximum irrelevances by $\hat{s}_{\max}\geq \hat{s}_1$ and $s^\st_{\max}$, we respectively obtained 
\begin{align*}
\log(\hat{s}_{\max})&\geq -(1-\gamma)(R/\Gamma)-\log T,\\
 -(R/\Gamma)-\log T\leq \log(s^\st_{\max})&\leq -(R/\Gamma)+\log T.
\end{align*}
The above inequalities satisfy Assumption \ref{asshurt} as follows where $\pb\gets\pb^\star_R$ and $\pb'\gets \pb_R$: Set $R_0=3\gamma^{-1}\Gamma\log T$ so that $\log T\leq \frac{\gamma R_0}{3\Gamma}$. Secondly, set $\rho_0=-(R_0/\Gamma)-\log T$. This way, $\rho_0\geq \log(s^\st_{\max})$ implies $R\geq R_0$ and $\log T\leq \frac{\gamma R}{3\Gamma}$. To proceed, using the latter inequality, we bound the $\log T$ terms to obtain
\begin{itemize}
\item $\log(\hat{s}_{\max})\geq -(1-2\gamma/3)(R/\Gamma)$.
\item $\log(s^\st_{\max})\leq -(1-\gamma/3)(R/\Gamma)$.
\end{itemize}
To proceed, we pick $1+\Delta=\frac{1-\gamma/3}{1-2\gamma/3}$ implying $\Delta:=\frac{\gamma}{3-2\gamma}$. Finally, for this $\Delta$, there exists $\rho(\Delta)$ which we need to ensure $\log(\hat{s}_{\max})\leq \rho(\Delta)$. This can be guaranteed by picking sufficiently large $R$ that ensures $\log(s^\st_{\max})\leq -(1-\gamma/3)(R/\Gamma)\leq \rho(\Delta)$ to satisfy all conditions of Assumption \ref{asshurt}. Since such large $R$ exists by initial assumption $\dist{\pbb_R, \Pc^\svm}\not\rightarrow0$, Assumption \ref{asshurt} in turn implies that $\Lc(\pb^\st_R)<\Lc(\pb_R)$ contradicting with the optimality of $\pb_R$ in \eqref{NPT loss}.
\end{proof}
% for sufficiently small $$ $R\geq R_0$ (which exists by initial assumption)
The following example will be further elaborated in Section \ref{sec:linear data} and shows that if irrelevant tokens result in label noise, Assumption \ref{asshurt} holds. The high-level idea behind this lemma is that, if the optimal risk is achieved by setting $\s^{\pb}_{\max}=0$, then, Assumption \ref{asshurt} will hold.%and $s_{\max}^{\pb}=\max_{i\in[n]}s^{\pb}_i$ 
\begin{lemma} [Linear label mixing] \label{label mix}Recall $s^{\pb}_i=\sum_{t\in \Rcb_t}\ab_{it}$ from Assumption \ref{asshurt}. Suppose $\link{\X_i^\top \ab_i}=\nu(1-s_i^{\pb})Y_i+Z_i$ for some $\nu> 0$. Here $Z_i$ is a zero-mean label-noise variable induced by the irrelevant tokens. For some $C>0$, $|Z_i|\leq Cs^{\pb}_{\max}$ for all $\pb$ (allowing for $Z_i=0$). Consider the expected loss over $Z_i$, namely, $\bar{\Lc}(\pb):=\E_{(Z_i)_{i=1}^n}[\Lc(\pb)]$. Then, Assumption \ref{asshurt} holds for $\bar{\Lc}(\pb)$ when either of the following conditions hold:
    \begin{itemize} 
        \item Suppose $\ell(\cdot)$ is the squared loss, labels $Y_i$ are arbitrary but nonzero, and $\nu\leq 1$.
        \item Suppose $\ell(\cdot)$ is the logistic loss, labels $Y_i\in\{-1,1\}$, and $\nu>0$ is arbitrary.
    \end{itemize}
\end{lemma}
\begin{proof} \noindent\textbf{$\bullet$ Case 1: squared loss.} Let us first consider the squared loss $(Y_i-\hat{Y}_i)^2$. Let $M_+=\max_{i\in[n]}Y_i^2,M_-=\min_{i\in[n]}Y_i^2>0$. Define $\Lc'(\pb):=\bar{\Lc}(\pb)-\frac{1}{n}\sum_{i=1}^n(1-\nu)^2Y_i^2$ where $\frac{1}{n}\sum_{i=1}^n(1-\nu)^2Y_i^2$ is the minimum achievable risk by setting $s_{\max}=0$ whenever $\nu\leq 1$. Using $\E[Z_i]=0$, we have that
%$\sigma_{\max}^2=\max_{i\in[n]}\sigma_i^2$%Denote $\E[Z_i^2]\leq C^2s_{\max}^2$
    \begin{align}
    \Lc'(\pb)&=\frac{1}{n}\sum_{i=1}^n\E_{Z_i}[(Y_i-\nu (1-s_i)Y_i-Z_i)^2]-\frac{1}{n}\sum_{i=1}^n(1-\nu)^2Y_i^2\\
    &= \frac{1}{n}\sum_{i=1}^n((1-\nu+\nu s_i)^2-(1-\nu)^2)Y_i^2+\E[Z_i^2]\\
    &=\frac{1}{n}\sum_{i=1}^n\nu s_i(2-2\nu+\nu s_i)Y_i^2+\E[Z_i^2]\\
    &\geq B:=\nu s_{\max}(2-2\nu+\nu s_{\max})M_-/n.
    \end{align}
    Using the identical argument and the upper bound $\E[Z_i^2]\leq C^2s_{\max}^2$, we also obtain an upper bound
    \[
    \Lc'(\pb)\leq \nu s_{\max}(2-2\nu+\nu s_{\max})M_++C^2s_{\max}^2.
    \]
    %$s_{\max}\leq 1$ and 
    Now, independent of the choice of $\pb$, the ratio of upper/lower bounds obey (using $\nu s_{\max}(2-2\nu+\nu s_{\max})\geq \nu s_{\max}^2$)
    \[
    \frac{\nu s_{\max}(2-2\nu+\nu s_{\max})M_++C^2s_{\max}^2}{B}\leq n\frac{M_++C^2/\nu}{M_-}:=\Theta.
    \] 
    %Recalling $s_{\max}:=\max_{i\in[n]}s_i$, clearly,
    %Setting $B:=(1-\nu+\nu s_{\max})\sqrt{M_-/n}$, 
    Overall, we found $\sqrt{\Theta}B\geq \sqrt{\Lc'(\pb)}\geq B$. Thus, for any $\pb,\pb'$, we have that, if $\sqrt{\Theta } s^{\pb}_{\max}(2-2\nu+\nu s^{\pb}_{\max})< s^{\pb'}_{\max}(2-2\nu+\nu s^{\pb'}_{\max})$, then $\Lcb(\pb)< \Lcb(\pb')$. Note that the former condition is implied by the stricter but cleaner criteria $\sqrt{\Theta } s_{\max}^{\pb}< s_{\max}^{\pb'}$.
    
    Going back to the condition of Assumption \ref{asshurt}, any $\log (s^{\pb}_{\max})\leq (1+\Delta)\log (s^{\pb'}_{\max})$ obeys $s^{\pb}_{\max}\leq (s^{\pb'}_{\max})^{1+\Delta}$ i.e. $s^{\pb'}_{\max}\geq (s^{\pb}_{\max})^{(1+\Delta)^{-1}}$. Following above, we wish to ensure $s^{\pb'}_{\max}>\sqrt{\Theta}s^{\pb}_{\max}$ for such $(\pb,\pb')$ pairs. This is guaranteed by
    \[
    (s^{\pb}_{\max})^{(1+\Delta)^{-1}-1}>\sqrt{\Theta}\iff \frac{\Delta}{1+\Delta}\log(s^{\pb}_{\max})< -0.5\log(\Theta).
    \]
    The above is satisfied by choosing a $\rho(\Delta):=-(1+\Delta^{-1})\log(\Theta)$ in Assumption \ref{asshurt}.

    \noindent\textbf{$\bullet$ Case 2: Logistic loss.} Logistic loss is relevant because (i) it is used in most classification problems and also (ii) softmax-attention and logistic loss are both exponential-tailed so their joint interaction is of practical interest for transformers. To proceed, let us write the logistic loss in a similar fashion where we use $\ell(Y,\hat{Y})=\ell(Y\hat{Y})=\log(1+e^{-Y\hat{Y}})$. Let $Z'_i=Y_iZ_i$ which is zero-mean with same variance. 
    \begin{align*}
        \bar{\Lc}(\pb)&=\frac{1}{n}\sum_{i=1}^n\E_{Z_i}[\ell(Y_i(\nu(1-s_i^{\pb})Y_i+Z_i))]\\
        &=\frac{1}{n}\sum_{i=1}^n\E_{Z_i}[\ell(\nu(1-s_i^{\pb})+Z'_i)].
        %&=\frac{-1}{2n}\sum_{i=1}^n[\log((1-s_i^{\pb})+s_i^{\pb} \eps)+\log((1-s_i^{\pb})-s_i^{\pb} \eps)]\\
        %&=\frac{-1}{2n}\sum_{i=1}^n\log((1-s_i^{\pb})^2-\eps^2s_i^{\pb})
        \end{align*}
    Compared to squared loss, here we describe a more general approach that leverage Lipschitzness under small perturbations. Pick a sufficiently small $\rho_0:=\rho_0(\nu)$ and assume $s_{\max}^{\pb}\leq \rho_0$. Then, for $|\gamma|\leq s_{\max}^{\pb}\leq \rho_0$, through Taylor series, we can write
    \[
    0\leq \ell(\nu+\gamma)-\ell(\nu)-\gamma\ell'(\nu)\leq \gamma^2\ell''(\nu).
    \]
    This implies the following upper/lower bounds on summands of $\bar{\Lc}(\pb)$ using $\E[Z_i]=0$, $|Z_i|\leq Cs_{\max}^\pb$, and convexity of $\ell(\nu)$
    \[
    0\leq \E_{Z_i}[\ell(\nu(1-s_i^{\pb})+Z'_i)]-\ell(\nu)+\nu s_i^{\pb}\ell'(\nu)\leq (\nu+C)^2s_{\max}^2.
    \]
    Set $\Lc'(\pb):=\Lc(\pb)-\ell(\nu)$ where $\ell(\nu)$ is the minimum achievable loss (thanks to the convexity of $\ell$). Since $\ell$ is strictly decreasing, $\Theta:=-\ell'(\nu)>0$. To proceed, we obtain
    \[
    (\nu+C)^2s_{\max}^2+\Theta\nu s_{\max}\geq \Lc'(\pb)\geq n^{-1}\Theta\nu s_{\max}.
    \]
    We now repeat the similar argument as squared loss: For any $\pb,\pb'$, we have that, if $(\nu+C)^2(s^{\pb}_{\max})^2+\Theta\nu s^{\pb}_{\max}< n^{-1}\Theta\nu s^{\pb'}_{\max}$, then $\Lcb(\pb)< \Lcb(\pb')$. Note that this condition is implied by the stricter but cleaner criteria $\bar{\Theta}s^{\pb}_{\max} < s^{\pb'}_{\max}$ with $\bar{\Theta}:=n(\Theta^{-1}\nu^{-1}(\nu+C)^2\rho_0+1)$ thanks to $s^{\pb}_{\max}\leq \rho_0$. Note that $\bar{\Theta}$ is independent of $\pb$ for any $s_{\max}^{\pb}\leq \rho_0$.

    Going back to the condition of Assumption \ref{asshurt}, any $\log (s^{\pb}_{\max})\leq (1+\Delta)\log (s^{\pb'}_{\max})$ obeys $s^{\pb}_{\max}\leq (s^{\pb'}_{\max})^{1+\Delta}$ i.e. $s^{\pb'}_{\max}\geq (s^{\pb}_{\max})^{(1+\Delta)^{-1}}$. Following above, we wish to ensure $s^{\pb'}_{\max}>\bar{\Theta}s^{\pb}_{\max}$ for such $(\pb,\pb')$ pairs. This is guaranteed by
    \[
    (s^{\pb}_{\max})^{(1+\Delta)^{-1}-1}>\bar{\Theta}\iff \frac{\Delta}{1+\Delta}\log(s^{\pb}_{\max})< -\log(\bar{\Theta}).
    \]
    The above is satisfied by choosing a $\rho(\Delta):=-2(1+\Delta^{-1})\log(\bar{\Theta})$ in Assumption \ref{asshurt}. Thus, setting $\rho=\min(\rho(\Delta),\log \rho_0)$, any $\log (s^{\pb}_{\max})\leq \rho$ satisfies the condition of Assumption \ref{asshurt} finishing the proof.
\end{proof}



%Let $\x_{i\alpha},\x_{i\beta}$ be arbitrary relevant and irrelevant tokens in $\X_i$ respectively. Suppose $\link{\x_{i\alpha}}=Y_i$ and $\link{\x_{i\beta}}=Z_i$ where $Z_i$ is the label-noise induced by the irrelevant tokens. Suppose $Z_i$ is random and for some $p,\eps>0$ $\P(Z_iY_i<-\eps)>p$. Then, Assumption \ref{asshurt} holds when $\ell$ is quadratic loss or for some there exists 
    %$allowed to be stochastic but there exists $ 
%\ab^\st_{it}
% To see this, consider the following optimization problem
% This implies that there exists $\eps>0$ such that $\tn{\pbb-\pb^\svm}\geq \eps$ for all $R\geq \delta^{-1}$. Now, consider the following optimization problem
    



%\begin{example}\label{linear example}\end{example}

==> sec/bc/single_05_15.tex <==
\section{Main Results with Linear Classifier Head}\label{linear head sec}
The goal of this section is to provide the optimization problem and identify conditions that lead to the implicit bias of softmax-attention with linear classifier head. The high-level intuition is that, in order for softmax-attention to exhibit implicit bias, the optimization problem should be forced to separate one tokens of the input sequence from the rest. 
%
% Let $\Sc=(Y_i,\X_i)_{i=1}^n$ denote the training dataset where $Y_i\in \{-1,1\}$ and $\X_i\in\R^{T\times d}$. For a loss function $\ell(\cdot):\R\rightarrow\R$, we consider \eqref{patt} with linear head $\vb$ by focusing on the following optimization objective %with logistic loss
%\begin{align}
%\Lc(\vb,\pb, \W)=\frac{1}{n}\sum_{i=1}^n \ell(Y_i\cdot\vb^\top\X_i^\top \sft{\W\X^\top \pb}).\label{lin det los}
%\end{align}

Throughout, we make the following assumption on the loss function: 

\begin{assumption}[Well-Behaved Losses]\label{assum:loss:prope} 
\hspace{-.1cm}%\textbf{.}
\vspace{-.1cm}
\begin{enumerate}[label={\textnormal{\textbf{A\arabic*.}}}, wide, labelwidth=!, labelindent=0pt]
\item\label{assu:ell:a1}~  $\ell$ is strictly decreasing and bounded from below.
\vspace{-.2cm}
\item\label{assu:ell:a2}~ $\ell^{\prime}$ is $M_0$-Lipschitz continuous and  $|\ell^{\prime}(u)|\leq M_1$ for all finite $u$.
\end{enumerate}
\end{assumption}
Variants of this assumption are very common in the literature on margin maximization and implicit bias \cite{soudry2018implicit,lyu2019gradient}. Assumption~\ref{assum:loss:prope} includes many common loss functions, including the logistic and exponential loss. Assumption \ref{assum:loss:prope} implies that $\mathcal{L}\left(\mathbf{p}\right)$ is a $\mc{O}\left((M_0+M_1) \smax^4\right)$-smooth function (see Appendix~\ref{app:conv:gd}), where $\bar{\sigma}_{\max}:= 1/n \sum_{i=1}^n \sigma_{\max}(\m{X}_i)$. For example, the exponential loss $\ell\left(u\right)=e^{-u}$ and the commonly used logistic loss $\ell\left(u\right)=\log\left(1+e^{-u}\right)$ both follow this assumption. 
%Much of our results are specific to optimizing $\pb$ given a fixed $\vb$. In this case, we will denote the loss function by $\Lc_{\vb}(\pb)$.
%\noindent\textbf{Regularized Path.} Given a  function $\Lc:\R^d\to\R$ 
%and an $\ell_2$-norm bound $R$, the regularized solution is defined as
%%\begin{align}\label{eq:reg_f}
%   $\pb(R):=\arg\min_{\|\pb\|\le R}\Lc(\pb)$.
%%\end{align}
%Note that $\pb(R)$ is not unique in general.
%
%\noindent\textbf{Gradient Descent.} 
%For gradient descent, we assume the  the objective $\Lc(\pb
%)$ is $L$-smooth and describe the gradient descent process as 
%\begin{equation}\label{eqn:GD}
%\pb(t+1) = \pb(t) - \eta(t) \nabla \Lc(\pb(t)),
%\end{equation}
%where $\eta(t)$ is the learning rate at time $t$ and $\nabla \Lc(\pb(t))$ is the gradient of $\Lc$ at $\pb(t)$.

We now introduce a convex hard-margin SVM problem that separates one token of the input sequence from the rest, jointly solved over all inputs. We will show that this problem captures the optimization properties of softmax-attention. Fix indices $\bal=(\alpha_i)_{i=1}^n$ and consider
\begin{align}
    \ps(\bal)=\arg\min_{\pb}\tn{\pb}\quad\text{subject to}\quad \min_{t\neq \alpha_i}\pb^\top(\kb_{i\alpha_i}-\kb _{it})\geq 1\quad\text{for all}\quad 1\leq i\leq n\tag{ATT-{SVM}}\label{attnsvm}.
\end{align}
%\noindent\textbf{Interpretation:} Each input $\X_i$ has an associated key matrix $\Kb$ with $T$ tokens $(\kb_{it})_{t=1}^T$. We aim to achieve the maximum margin $m_i$ in order to separate the single best \rel token from all \irel tokens. Additionally, we wish to accomplish this goal for all inputs in the dataset, thus, we need to find the best $\pb$ that ensures all margins obey $m_i\geq 1$.
%When $\bal$ is clear from context, we will denote the solution by $\ps$. 
%The contribution of an individual token to the loss function is captured by its score $\bgam_{it}:=Y_i\cdot \vb^\top\x_{it}$. %Note that, score vector $\bgam_i=\X_i\vb\in\R^T$ is the value embeddings of the input features.
%For clearer discussion, we assume token scores are distinct (which holds for almost all datasets).
%\noindent\textbf{.}

The optimal tokens that achieve the smallest training objective under decreasing loss function $\ell(\cdot)$ have a clear definition:


\begin{definition}[Optimal Tokens]
The optimal tokens $\xbo_i$ for each input $\X_i$ are those tokens with highest scores given by
\[
\op_i\in\arg\max_{t\in [T]}Y_i\cdot\vb^\top \x_{it}.
\] 
\end{definition}
We denote the solution of \eqref{attnsvm} with optimal indices $(\op_i)_{i=1}^n$ by $\pso$. Note that multiple tokens within an $\X_i$ might attain same score, thus $\op_i$ and $\pso$ may not be unique.
% or simply $\ps$ when it is clear from context.





\subsection{Global Convergence on Attention Weights $\pba$}\label{sec linear p}
In this section, we state the main result of this paper, which characterizes the implicit bias
of gradient descent on learning $\pb$ and operates with a fixed $\vb\in\R^d$. 

To proceed with our global convergence analysis, we need to make the assumption that all non-optimal tokens have equal scores. In other words, if a potential solution includes tokens that do not appear in the final optimal solution, all of these tokens are assumed to have the same score value.

\begin{assumption}\label{assum:opt:token}
If for all $i\in[n]$ and $t_1,t_2\neq \op_i$, $\vb^\top \x_{it_1}=\vb^\top \x_{it_2}<\vb^\top \x_{i\op_i}$
\end{assumption}


 
\begin{theorem}[Global Convergence of Gradient Descent]\label{conv:gd:global}
Suppose Assumption~\ref{assum:loss:prope} on the loss function $\ell$ and Assumption \ref{assum:opt:token} on the tokens' score hold. Then the gradient descent iterates $\pb(t+1) = \pp{t} - \eta \nabla \Lc_{\pb}(\pb(t))$, with the step size $\eta \leq \mc{O}\left(\bar{\sigma}_{\max}^{-4} /(M_0+M_1)\right)$ and any starting point $p(0)$ satisfies $\lim_{t\rightarrow\infty}\pb(t)/\|\pb(t)\|=\pso/\tn{\pso}$.
\end{theorem}
\begin{proofsk}
We first show that under Assumption~\ref{assum:opt:token}, the gradient of training loss \eqref{lin det losss} satisfies $-\li\nabla\Lc(\pb),\pso\ri > 0$ for all $\pb\in\R^d$. This, combined with Assumption~\ref{assum:loss:prope}, implies that $\lim_{t\rightarrow\infty}\left\Vert \mathbf{p}\left(t\right)\right\Vert =\infty$.

Next, we establish that for any $\epsilon \in (0,1)$, there exists $t_0 \in \mb{N}$ such that for all $t\geq t_0$, the iterates of the gradient descent satisfy:
\begin{align*}
\iprod{-\nabla\mc{L}(\pb(t))}
     {\frac{\pso}{\|\pso\|}} \geq (1-\epsilon)\iprod{-\nabla \mc{L}(\pb(t))}{\frac{\pb(t)}{\|\pb(t)\|}}.
\end{align*}

Moreover, the gradient descent method with an appropriate step size guarantees a sufficient decrease of the smooth objective function after a single step: $\mc{L}(\pb({t+1}))-\mc{L}(\pb(t))\leq- \eta/2 \|\nabla \mc{L}(\pb(t))\|^2$. Combining this inequality with the aforementioned inequality, we obtain:
\begin{align*}
\left \langle \frac{\pb(t+1)}{\|\pb(t+1)\|},\frac{\pso}{\|\pso\|} \right \rangle\ge  1-\epsilon
%\frac{\left\langle \pb_{t_0}, \frac{\pso}{\|\pso\|}\right\rangle-(1-\epsilon)\|\pb_{t_0}\| -\eta (\mc{L}(\pb_{t_0})-\mc{L}^*)}{\|\pb(t+1)\|}
+\mc{O}\left(\frac{\eta \left(\mc{L}(\pb(t_0))- \min_{\pb}\mc{L}(\pb)\right)}{\|\pb(t)\|}\right).
    \end{align*}
Since $\epsilon \in (0,1)$ can take any value within this range, we conclude that $\lim_{t\rightarrow\infty}\pb(t)/\|\pb(t)\|=\pso/\tn{\pso}$.
%We first show that under Assumption~\ref{assum:opt:token}, for all $\pb\in\R^d$, the training loss \eqref{lin det losss} obeys 
%$-\li\nabla\Lc(\pb),\pso\ri > 0$. This together with  Assumption~\ref{assum:loss:prope} implies that $\lim_{t\rightarrow\infty}\left\Vert \mathbf{p}\left(t\right)\right\Vert =\infty$. 
%We then show that for any  $\epsilon \in (0,1)$, there exists $t_0 \in \mb{N}$ such that for all $t\geq t_0$ the gradient descent iterates satisfy
%\begin{align*}
%\iprod{-\nabla\mc{L}(\pb(t))}
%     {\frac{\pso}{\|\pso\|}} \geq (1-\epsilon)\iprod{-\nabla \mc{L}(\pb(t))}{\frac{\pb(t)}{\|\pb(t)\|}}.
%\end{align*}
%On the other hand, gradient descent method with proper step size provides sufficient decrease of the smooth objective function after a single step, i.e., $\mc{L}(\pb({t+1}))-\mc{L}(\pb(t))\leq- \eta/2 \|\nabla \mc{L}(\pb(t))\|^2$. This together with the above inequality gives 
%\begin{align*}
%\left \langle \frac{\pb(t)}{\|\pb(t)\|},\frac{\pso}{\|\pso\|} \right \rangle\ge  1-\epsilon
%%\frac{\left\langle \pb_{t_0}, \frac{\pso}{\|\pso\|}\right\rangle-(1-\epsilon)\|\pb_{t_0}\| -\eta (\mc{L}(\pb_{t_0})-\mc{L}^*)}{\|\pb(t)\|}
%+\mc{O}\left(\frac{\eta (\mc{L}(\pb(t_0))- \mc{L}^*)}{\|\pb(t)\|}\right).
%    \end{align*}
%As $\epsilon \in (0,1)$ can take any value within that range, we obtain $\lim_{t\rightarrow\infty}\pb(t)/\|\pb(t)\|=\pso/\tn{\pso}$.
\end{proofsk}
%\begin{assumption} \label{distinct ass}Let $\bgam_i=\X_i\vb\in\R^T$ be the score function of input $i$. The entries of $\bgam_i$ are distinct for $i\in[n]$.
%\end{assumption}


Theorem~\ref{conv:gd:global} presents compelling evidence that gradient descent optimization of \eqref{lin det losss} with respect to $\pb$ leads to the convergence of the normalized predictor $\pb(t)/\|\pb(t)\|$ towards $\pso/\tn{\pso}$, effectively separating globally optimal tokens from non-optimal ones. To illustrate this theorem, we can refer to Figure \ref{fig:global}. In the figure, the gray paths represent gradient descent trajectories initiated from different points, while the points $(0,0)$ and $(1,0)$ correspond to non-optimal tokens, and $(-.1,1)$ represents the optimal token. Notably, gradient descent iterates with various starting points converge towards the direction of the max-margin solution $\pso$ (depicted by {\color{red}-~-~-}). Moreover, as the iteration count $t$ increases, the inner product $\left \langle \pb(t)/\|\pb(t)\|,\pso/\|\pso\| \right \rangle$ consistently increases. This observation emphasizes the gradual alignment between the evolving predictor and the max-margin solution throughout the optimization process.

We next provide the regularization path analysis that requires relaxed assumptions on both loss function and tokens' score.

\begin{theorem}[Regularization Path]\label{lin det thm} Suppose Assumption~\ref{assu:ell:a1} on the loss function hold,  and  for all $i\in[n]$ and $t\neq \op_i$, $\vb^\top \x_{it}<\vb^\top \x_{i\op_i}$. Then the regularization path $\pr{R}=\arg\min_{\tn{\pb}\leq R}\Lc(\pb)$  %of \eqref{lin det los}. 
satisfies $\lim_{R\rightarrow\infty}\pr{R}/R=\pso/\tn{\pso}$.
% with logistic loss and gradient descent converges to the \eqref{svm} solution $\ps/\tn{\ps}$ with $\Rc_i=\{\alpha_i\}$.%Set $\Kb_i=\W^\top\X_i$. 
\end{theorem}

Theorem~\ref{lin det thm} reveals that as we loosen the regularization strength $R$ to achieve ridgeless optimization with $\min_{\pb}\Lc(\pb)$, the optimal direction $\pr{R}$ gradually aligns with the max-margin solution $\pso$. It is worth noting that unlike Theorem~\ref{conv:gd:global}, this theorem does not necessitate the presence of a $M_0$-smooth loss function with a bounded gradient. Furthermore, an important distinction of this theorem is its ability to handle non-optimal tokens that possess different scores.

%\begin{assumption}\label{assum:loss:prope}
%The loss function $\ell(u)$ is strictly decreasing, bounded from below, $M_0$-smooth, $\lim\sup_{u\rightarrow-\infty}\ell^{\prime}\left(u\right)<0$, and  $|\ell^{\prime}(u)|\leq M_1$ for all finite $u$.
%\end{assumption}
%Assumption~\ref{assum:loss:prope} includes many common loss functions, including the logistic, exp-loss, %\footnote{The exp-loss does not have a global $\beta$ smoothness parameter. However, if we initialize with $\eta < 1/ \mathcal{L}(\pb(0))$ then it is straightforward to show the gradient descent iterates maintain bounded local smoothness.} 
%and probit losses. Assumption \ref{assum:loss:prope} implies
%that $\mathcal{L}\left(\mathbf{p}\right)$ is a $\mc{O}\left((M_0+M_1) \bar{\sigma}_{\max}^4\right)$-smooth function (see Appendix~\ref{app:conv:gd}), where $\bar{\sigma}_{\max}:= 1/n \sum_{i=1}^n \sigma_{\max}(\m{X}_i)$. For example, the exponential loss $\ell\left(u\right)=e^{-u}$ and the commonly used logistic loss $\ell\left(u\right)=\log\left(1+e^{-u}\right)$
%both follow this assumption. Note that we do not require convexity. 
%
%\\&\geq \frac{(\bgam_1-\gamma)}{1-\s_1} \abg>0.
% (in terms of verifying) and we can focus on only.
%\begin{lemma}[Local descent conditions] 
%\end{lemma}
%and fixed $\vb$. This loss obeys conditions of Lemma \ref{label mix}. Thus, per Theorem \ref{meta thm}, the regularization path $\pb_R/R$ of \eqref{lin det los} 
%\begin{theorem}\label{lin det thm}\red{[SIMPLE BUT CORRECT]} Suppose classifier head $\vb\in\R^d$ is such that, for all inputs $i\in[n]$, it obeys
%\[Y_i\cdot\vb^\top \x_{i1}>|\vb^\top \x_{it}|,\quad\forall t\geq 2.\]
%Set $\Kb_i=\W^\top\X_i$. Consider \eqref{lin det los} with logistic loss and fixed $\vb$. This loss obeys conditions of Lemma \ref{label mix}. Thus, per Theorem \ref{meta thm}, the regularization path $\pb_R/R$ of \eqref{lin det los} converges to an \eqref{svm} solution $\ps/\tn{\ps}$.
%\end{theorem}





\subsection{ Local Convergence on Attention Weights $\pba$}
In this section, we discuss the local convergence of gradient descent methods towards the max margin solution in the context of Attention SVM. Our theory builds on two new concepts: locally-optimal tokens and neighbors of tokens. 
%\begin{theorem}\label{local det thm} Fix a vector $\vb\in\R^d$. Define scores $\bgam_i=\X_i\vb$. Suppose gradient descent on $\pb$ achieves a limit $\pb^\star=\pb_t/\tn{\pb_t}$. Suppose $\lim_{t\rightarrow\infty}\sft{\Kb_i\pb_t}$ are one-hot vectors (selects only one token). Then, there exists indices $(\alpha_i)_{i=1}^n$ such that, $\pb^\star=\ps/\tn{\ps}$ where $\ps$ is the SVM solution
%\begin{align}
%\ps=\arg\min_{\pb\in\R^d} \tn{\pb}\quad\text{subject to}\quad \pb^\top (\kb_{i\alpha_i}-\kb_{it})\geq 1\label{svm-local}.
%\end{align}
%Additionally, in this SVM, all support vectors $\x_{it}$ obeying $\pb^\top (\x_{i\alpha_i}-\x_{it})=1$ satisfy $\bgam_{it}<\bgam_{i\alpha_i}$.
%\end{theorem}
%\begin{assumption} [\neis have same score]\label{assum:regular} Fix token indices $\bal=(\alpha_i)_{i=1}^n$ and let $\Tc_i\subset[T]$ be their \neis for $i\in[n]$. For all $i\in[n]$ and $t_1,t_2\in\Tc_i$, the scores are same, i.e., $\x_{it_1}^\top\vb=\x_{it_1}^\top \vb$.
%% Relaxing this assumption is tricky because there are $\pb$ directions with gradients subpar correlations with $\ps$. The reason is that $\pb$ can select the lowest score neighbor to get high-corr whereas $\ps$ will be $\Omega(1)$ less corr.
%\end{assumption}



\begin{definition}[SVM-Neighbor and Locally-Optimal Tokens]\label{def loc opt} Fix token indices $\bal=(\alpha_i)_{i=1}^n$. Solve \eqref{attnsvm} to obtain $\ps=\ps(\bal)$. Consider tokens $\Tc_i\subset[T]$ such that $(\kb_{i\alpha_i}-\kb_{it})^\top \ps=1$ for all $t\in\Tc_i$. We refer to $\Tc_i$ as \neis of $\kb_{i\alpha_i}$. Additionally, tokens $\bal=(\alpha_i)_{i=1}^n$ are called locally-optimal if for all $i\in[n]$, $t\in\Tc_i$, we have that $\vb^\top (\x_{i\alpha_i}-\x_{it})>0$. 
\end{definition}
%
%\begin{assumption} [\neis have same score]\label{assum:regular} Fix token indices $\bal=(\alpha_i)_{i=1}^n$ and let $\Tc_i\subset[T]$ be their \neis for $i\in[n]$. For all $i\in[n]$ and $t_1,t_2\in\Tc_i$, the scores are same, i.e., $\x_{it_1}^\top\vb=\x_{it_1}^\top \vb$.
%% Relaxing this assumption is tricky because there are $\pb$ directions with gradients subpar correlations with $\ps$. The reason is that $\pb$ can select the lowest score neighbor to get high-corr whereas $\ps$ will be $\Omega(1)$ less corr.
%\end{assumption}

To provide a basis for discussing local convergence, we establish a cone centered around $\ps$ using the following construction. Let $\mu$ be a positive scalar, and define the cone as:

\begin{equation}\label{eqn:def:cone}
\cone_{\mu}(\ps) := \left\{ \pb \Big| \left\langle\frac{\pb}{\|\pb\|},\frac{\ps}{\|\ps\|} \right\rangle\geq 1-\mu\right\}.
\end{equation}

In the subsequent theorem, we demonstrate the existence of a scalar $\mu=\mu(\bal)>0$ and a radius $R$ such that when $R$ is sufficiently large, there are no stationary points within the intersection of $\cone_{\mu}(\ps)$ and the set $\left\{\pb~|~\tn{\pb}\geq R\right\}$. Further, the gradient descent initialized within this intersection converges in direction to $\ps/\|\ps\|$.

% $\cone_{\mu}(\ps) $ that is devoid of stationary points of $\mc{L}(\pb(t))$, and standard gradient methods converge towards the max margin solution, as long as they are initialized within this cone.% $\cone_{\mu,R}(\ps)$ for some $\mu$.
\begin{theorem}[Local Convergence of Gradient Descent]\label{thm:local:gd} 
 Suppose  Assumption~\ref{assum:loss:prope} on the loss function $\ell$ hold and  assume $\bal=(\alpha_i)_{i=1}^n$ are locally-optimal tokens per Definition \ref{def loc opt}.  Then, there exists a scalar $\mu=\mu(\bal) \in (0,1)$ and a radius $R>0$ such  that   $\cone_{\mu}(\ps)\bigcap \left\{\pb~|~\tn{\pb}\geq R\right\}$  does not contain any  stationary points. Further, the gradient descent iterates
$\pb(t+1) = \pp{t} - \eta \nabla \Lc(\pb(t))$ with
\begin{align}\label{eqn:step:loc}
\eta \leq \mc{O}  \left(\min\left(\frac{1}{(M_0+M_1) \bar{\sigma}^4_{\max}}, \frac{\mu-\epsilon }  {(1-\mu)\|\nabla \mc{L}(\pb(t))\|^2}\right)\right),    
\end{align}
for any $\epsilon \in (0, \min(\mu,1))$, and any starting point $p(0) \in  \cone_{\mu}(\ps)\bigcap \left\{\pb~|~\tn{\pb}\geq R\right\}$  satisfies $\lim_{t\rightarrow\infty}\pb(t)/\|\pb(t)\|=\ps /\|\ps \|$. 
\end{theorem}    
\begin{proofsk}
We provide the proof in four steps:\\
\textbf{Step~1.} We begin by proving that there are no stationary points within  $\cone_{\mu}(\ps)\bigcap \left\{\pb~|~\tn{\pb}\geq R_m\right\}$  for a specific radius $R_\mu$. Let $(\Tc_i)_{i=1}^n$ denote  the set of SVM-neighbors as defined in Definition \ref{def loc opt}. We define $\Tcb_i=[T]-\Tc_i-{\alpha_i}$ as the tokens that are non-SVM neighbors. Additionally, let
\begin{equation*}%\label{eqn:local:mu}
\begin{split}
&\Theta:=\frac{1}{\tn{\ps}},~~\delta:=\frac{1}{2}\min_{i\in[n]}\min_{t\in\Tc_i,\tau\in\Tcb_i}(\kb_{it}-\kb_{i\tau})^\top \ps,\\
A&:=\max_{i\in[n],t\in[T]}\tn{\kb_{it}}\tn{\ps},~~
\mu:=\frac{1}{8}\left(\frac{\min(0.5,\delta)}{A}\right)^2.
%\Gamma&=\sup_{i\in[n],t,\tau\in[T]}|\bgam_{it}-\bgam_{i\tau}|,
\end{split}
\end{equation*}
For all $\qb,\pb\in \cone_{\mu}(\ps)$ with $\tn{\qb}=\tn{\ps}$, we establish the existence of $R_\mu$ such that $-\qb^\top \nabla \Lc(\pb)$ is strictly positive for $\tn{\pb}\geq R_\mu$. Specifically, we show the existence of positive constants $C$ and $c$ satisfying:
\begin{align*}
C\cdot\max_{i\in[n]}q_i \geq -\li\nabla\Lc(\pb),\qb\ri\geq c\cdot\min_{i\in[n]}q_i>0. %\label{local simplified bound}
\end{align*}
Here,  $q_i=1-\sft{\Kb_i\pb}_{\alpha_i}$ and $\bal=(\alpha_i)_{i=1}^n$ are locally-optimal tokens per Definition \ref{def loc opt}.  

%\textbf{There is no stationary point within $\cone_{\mu}(\ps)\bigcap \{\pb\bgl\tn{\pb}\geq R\}$ for some $R=R_\mu$}.
\textbf{Step~2.}  We demonstrate that for any $\epsilon \in  (0, \min(\mu,1))$, there exists $R_\epsilon$ such that all $\pb\in \cone_{\mu}(\ps)\bigcap \{\pb~|~\tn{\pb}\geq R_\epsilon\}$ satisfy
\begin{align*}
\iprod{-\nabla\mc{L}(\pb)}{\frac{\ps}{\|\ps\|}} \geq (1-\epsilon)\iprod{-\nabla \mc{L}(\pb)}{\frac{\pb}{\|\pb\|}}.
\end{align*}
\textbf{Step~3.}
By leveraging the results from \textbf{Step 1} and \textbf{Step 2}, we can demonstrate that the gradient iterates, with an appropriate step size, starting from $p(0) \in \cone_{\mu}(\ps)\bigcap \{\pb~|~\tn{\pb}\geq R\}$, remain within this cone. Specifically, if $ p(t) \in \cone_{\mu}(\ps)\bigcap \{\pb~|~\tn{\pb}\geq R\}$, then $\|\pb(t+1)\| \geq \|\pb(t)\|$, and
\begin{equation*}
\begin{split}
\left\langle \frac{\pb(t+1)}{\|\pb(t+1)\|},\frac{\ps}{\|\ps\|} \right\rangle \geq 1-\mu+ \mc{O}\left(\eta(\mu -\epsilon)\right). 
\end{split}
\end{equation*}
which implies that, with the step size $\eta$ satisfying \eqref{eqn:step:loc}, $\pb(t+1)$ remains in $\cone_{\mu}(\ps)\bigcap \{\pb~|~\tn{\pb}\geq R\}$.

\textbf{Step~4.} The remaining part of the proof follows the same reasoning as the proof of Theorem~\ref{conv:gd:global}.
\end{proofsk}

To further illustrate Theorem~\ref{thm:local:gd}, we can consider Figure \ref{fig:local} where $n=1$ and $T=3$. In this figure, the point $(0,0)$ represents the non-optimal tokens, while $(1,0)$ represents the locally optimal token. Additionally, the gray paths represent the trajectories of gradient descent initiated from different points. By observing the figure, we can see that gradient descent, when properly initialized, converges towards the direction of $\ps$ (depicted by {\color{blue}-~-~-}). This direction of convergence effectively separates the locally optimal tokens $(1,0)$ from the non-optimal token $(0,0)$.

Let $\bal=(\alpha_i)_{i=1}^n$ be locally-optimal tokens per Definition \ref{def loc opt}. Let $(\Tc_i)_{i=1}^n$ be the set of all \neis per Definition \ref{def loc opt}, and $\Tcb_i=[T]-\Tc_i-\{\alpha_i\}$ be the non-SVM-neighbor tokens. Consider the conic set that strictly prioritizes neighbor tokens over non-neighbor tokens% $\pb$ obeying
\begin{equation}
\overline{\texttt{cone}}_{\epsilon,\Xi}(\bal):=\left\{\pb~\Big|~\min_{i\in[n]}\max_{t\in\Tc_i}\min_{\tau\in\Tcb_i}\pb^\top(\kb_{it}-\kb_{i\tau})/\tn{\pb}\geq \eps,~\tn{\pb}\geq \Xi\right\}.
\end{equation}

%The following theorem shows that the regularized path of 
%
\begin{theorem} [Local Regularization Path]\label{local path theorem} Fix locally-optimal token indices $\bal=(\alpha_i)_{i=1}^n$ with \neis $(\Tc_i)_{i=1}^n$. %Fix $\Xi,\eps>0$.
%Define the local regularization path $\prl{R}=\min_{\text{cone}(\bal),\tn{\pb}\leq R}\Lc(\pb)$.
For any $\eps>0$ and sufficiently large $\Xi= O(1/\eps)>0$, the  local regularization path $\prl{R}=\min_{\cone(\bal),\tn{\pb}\leq R}\Lc(\pb)$ satisfies $\lim_{R\rightarrow\infty} \prl{R}/R=\ps(\bal)/\|\ps(\bal)\|$.
\end{theorem}
\noindent \textbf{Remark.} This theorem is tight in the sense that, as soon as $\bal$ is not locally-optimal (as detailed in Lemma \ref{lem not optimal}), the limit will not converge to $\ps(\bal)$.

\begin{lemma}\label{lem not optimal} Consider the setting of Theorem \ref{local path theorem}. However, suppose $\bal$ is not locally-optimal and has an \nei $\bet\in\R^n$ with $\beta_i\in\Tc_i$ achieving strictly better risk as follows 
\[
\sum_{i=1}^n \ell(\bgam_{i\beta_i})<\sum_{i=1}^n \ell(\bgam_{i\alpha_i}).
\]
Additionally assume \eqref{attnsvm} with $\bet$ is separable (i.e.~$\pb(\bet)$ exists). Then the limit of the local regularization path over $\text{cone}(\bal)$ will not converge to $\ps(\bal)$.
\end{lemma}


==> sec/contextual.tex <==
%We will use a semi-random model where contextual features are deterministic whereas label is stochastic.

\section{Contextual Dataset with Linear Heads}
The goal of this section is providing a tangible example that obeys Lemma \ref{label mix}. Consider the following dataset definition that builds on the discussion above. Let $\onebb_{X}$ denote the indicator function of a boolean $X$.
\begin{assumption} [Linear head setting] \label{asslin} Fix $Y_i\in\{-1,1\}$. Fix vectors $\vstar\in\R^d$ and $\cb_{it}\in\R^d$ for $i\in [n],t\in[T]$. The tokens of the $i$'th input obeys
\begin{align}
\x_{it}=\cb_{it}+\onebb_{t\in \Rc_{i}} Y_i\cdot \vstar.\label{LDM}%\tag{LINSEP}
\end{align}
\end{assumption}

%Let $\vstab\in\R^d$ be the projection of $\vstar$ on the orthogonal complement of $(\cb_{it})_{i,t\geq 1}$ and assume $\vstab\neq 0$. 
\begin{theorem}\label{lin det thm2}\red{[SIMPLE BUT CORRECT]} Suppose Assumption \ref{asslin} holds and pick $\vstab\in\R^d$ to be the projection of $\vstar$ on the complement of $(\cb_{it})_{i,t\geq 1}$'s. Set $\Kb_i=\W^\top\X_i$. Consider the training risk with logistic loss
    \begin{align}
    \Lc(\pb)=\frac{1}{n}\sum_{i=1}^n \ell(Y_i\vstab^\top\X_i^\top \sft{\Kb_i\pb}).\label{lin det loss2}
    \end{align}
    This loss obeys conditions of Lemma \ref{label mix}. Thus, per Theorem \ref{meta thm}, the regularization path $\pb_R/R$ of \eqref{lin det loss2} converges to an \eqref{svm} solution $\pb^\svm/\tn{\pb^\svm}$.
\end{theorem}
\begin{theorem}\label{lin det thm3} Suppose Assumption \ref{asslin} holds and pick $\vstab\in\R^d$ such that $\sup_{i,t}|\vstab^\top \cb_{it}|<\vstab^\top\vstar$. Set $\Kb_i=\W^\top\X_i$. Consider the training risk with logistic loss
    \begin{align}
    \Lc(\pb)=\frac{1}{n}\sum_{i=1}^n \ell(Y_i\vstab^\top\X_i^\top \sft{\Kb_i\pb}).\nn
    \end{align}
    This loss obeys conditions of Lemma \ref{label mix}. Thus, per Theorem \ref{meta thm}, the regularization path $\pb_R/R$ of \eqref{lin det loss2} converges to an \eqref{svm} solution $\pb^\svm/\tn{\pb^\svm}$.
\end{theorem}
\begin{proof} Set $\ab_i=\sft{\Kb_i\pb}$. Let $\vstab^\top\vstar=\nu>0$ and $\nu':=\sup_{i,t}|\vstab^\top \cb_{it}|<\nu$. We find 
\[
\hat{Y}=\vstab^\top\X_i^\top \ab_i=\sum_{t\in[T]}\vstab^\top \x_{it}\ab_{it}=\sum_{t\in\Rc_i}\nu Y_i\ab_{it}+\sum_{t\in[T]} \vstab^\top\cb_{it}\ab_{it}=\nu Y_i(1-s^{\pb}_i)+Z_i.
\]
Here, we set $Z_i:=\sum_{t\in[T]} \vstab^\top\cb_{it}\ab_{it}$. Note that $|Z_i|\leq \sum_{t\in\Rcb_i}\nu'\ab_{it}\leq \Gamma\nu s_i^{\pb}$ with $\Gamma=\nu'/\nu<1$.
Thus, conditions of Lemma \ref{label mix} holds. Applying this lemma, we conclude.
\end{proof}



\subsection{Stochastic Noise}
The following result applies under zero-mean label noise. However, it can address the scenario where label-noise $Z_{it}$ is (much) larger than the label strength $Y_i$ to cause classification error.
\begin{assumption} [Linear head -- Stochastic] \label{asslin2} Fix $Y_i\in\{-1,1\}$. Let $(Z_{i})_{i}^n$ be zero-mean variables bounded by some $\Gamma>0$. Fix vectors $\vstar\in\R^d$ and $\cb_{it}\in\R^d$ for $i\in [n],t\in[T]$. The tokens of the $i$'th input obeys
    \begin{align}
    \x_{it}=\cb_{it}+(\onebb_{t\in \Rc_i}Y_i+\onebb_{t\in \Rcb_i}Z_i)\vstar.\label{LDMS}
    %\begin{cases}Y_i\cdot\vstar\quad t\in \Rc_{\X}\\Z_{i}\cdot\vstar\quad t\in \bar{\Rc}_{\X}\end{cases}.\tag{LINSEP}
    \end{align}
    \end{assumption}
\begin{theorem}\label{lin path thm} Suppose Assumption \ref{asslin2} holds. Let $\vstab\in\R^d$ be the projection of $\vstar$ on the orthogonal complement of $(\cb_{it})_{i,t\geq 1}$. Consider the training risk with logistic loss
\begin{align}
\Lc(\pb)=\frac{1}{n}\sum_{i=1}^n \E_{Z_i}[\ell(Y_i\vstab^\top\X_i^\top \sft{\Kb_i\pb})].\label{LPT loss}
\end{align}
This loss obeys the conditions of Lemma \ref{label mix}. Thus, its regularization path $\pb_R/R$ converges to an \eqref{svm} solution $\pb^\svm/\tn{\pb^\svm}$ over the key distribution $(\kb_{it})_{i,t\geq 1}$. That is, we solve \eqref{svm} over the union of key features $(\Kb_i)_{i\in[n]}$ induced by the noise realizations $(Z_i)_{i\in [n]}$.
\end{theorem}% (whenever the \eqref{svm} is solvable)
%\textbf{Remark:} Note that, if the problem is noiseless, then we converge to the \eqref{svm} solution with $(\kb_{it})_{i,t\geq 1}$. However, adding stochastic noise has the affect of generating a larger dataset, thus, the statement of the theorem accounts for this distributional nature.

\begin{proof} Set $\ab_i=\sft{\Kb_i\pb}$. Let $\vstab^\top\vstar=\nu>0$. Observe that, since $\vstab$ is orthogonal to contexts, we find 
\[
\hat{Y}=\vstab\X_i^\top \ab_i=\sum_{t\in[T]}\vstab \x_{it}\ab_{it}=\sum_{t\in\Rc_i}\nu Y_i\ab_{it}+\sum_{t\in\Rcb_i}\nu Z_i\ab_{it}=\nu Y_i(1-s^{\pb}_i)+\nu Z_is^{\pb}_i.
\]
Since $Z_i$ is zero-mean and bounded by constant, conditions of Lemma \ref{label mix} holds. Applying this lemma, we conclude.
\end{proof}

The lemma below shows that \eqref{svm} solution actually has a simple distribution-agnostic solution when the key embeddings of $\vstar$ and $\cb_{it}$ are orthogonal. This simplifies the statement of the previous theorem.
%Suppose label $Y_i\in \{-1,1\}$ and noise $Z_i$ are independent and zero-mean for $i\in[n]$.
\begin{lemma}[Closed form under orthogonality] Let $Y_i-Z_i$ be discrete random variables that admit both positive and negative values for $i\in[n]$. Suppose $\W^\top\vstar$ is orthogonal to $\kbb_{it}=\W^\top\cb_{it}$ for all $i,t\geq 1$.
%Let $\kbb_{it}$ be the projection of $\kb_{it}=\W^\top\x_{it}$ on the orthogonal complement of $\W^\top\vstar$. 
% are orthogonal under mild distributional assumptions
Then, the regularization path $\pb_R/R$ of $\Lcb(\pb)=\E_{Y_i,Z_i}[\Lc(\pb)]$ (adapting \eqref{lin det loss2}) converges to a $\pb^\svm/\tn{\pb^\svm}$ obtained by \eqref{svm} over the keys $(\kbb_{it})_{i,t\geq 1}$.
\end{lemma}
% where $\x_{it}=\cb_{it}+\{Y_i,Z_i\}\vstar$%(valueless) 
\begin{proof} Let $\vstab=\W^\top\vstar$. Applying Theorem \ref{lin path thm}, we know that regularization path converges to an \eqref{svm} solution $\pb_1$ over the key distribution $\kb_{it}=\kbb_{it}+\{Y_i,Z_i\}\vstab$. Let $\pb_2$ be an \eqref{svm} solution over orthogonalized $\kbb_{it}$. We will show $\pb_1,\pb_2$ are equivalent. First, due to orthogonalization, we have that $\pb_2^\top\vstab=0$.

Secondly, let $\pb_1=\pb'_1+\pb^\perp_1$ where $\pb^\perp_1$ is the projection of $\pb_1$ on $\vstab$ direction. Given $\alpha\in\Rc_i,\beta\in\Rcb_i$, using orthogonality of $\kbb_{it},\vstab$, we have 
\[
\pb_1^\top(\kb_{i\alpha}-\kb_{i\beta})=(\kbb_{i\alpha}-\kbb_{i\beta})^\top\pb'_1+(Y_i-Z_i)\vstab^\top \pb^\perp_1.
\]
To proceed, we claim that $\pb^\perp_1= 0$. Otherwise, assume $\vstab^\top \pb^\perp_1>0$ (without losing generality). For fixed context vector $(\cb_{it})_{i,t\geq 1}$ choices, find the label-noise realization $(Y',Z')$ such that the variable $Y_i-Z_i$ attains its minimum value. $Y'-Z'\leq -\kappa$ for some $\kappa>0$ thanks to the positive-negative value assumption. Observe that $\x_{it}=\cb_{it}+\{Y',Z'\}\vstar$ is the input realization that achieves the minimum margin (for each fixed $\{\cb_{it}\}$ choice) due to $\vstab^\top \pb^\perp_1>0$. Let $(\alpha,\beta)$ be the token indices achieving this margin (for fixed $\{\cb_{it}\}$). Since $(Y'-Z')\vstab^\top \pb^\perp_1\leq -\kappa\vstab^\top \pb^\perp_1<0$, picking $\pb'_1$ in \eqref{svm} yields a margin lower bound $(\kbb_{i\alpha}-\kbb_{i\beta})^\top\pb'_1\geq 1+\kappa\vstab^\top \pb^\perp_1>1$ for all realizations of $(Y_i,Z_i)$. Consequently, choosing $\pb'_1$ rather than $\pb_1$ leads to strictly better overall margin (by improving all negative $Y_i-Z_i$ realizations). This contradicts with the optimality of $\pb_1$. 

Thus $\pb^\perp_1=\pb_1^\top\vstab=0$. With this established, observe that SVM margin constraints of $\pb_1$ are now only in terms of $\pb_1^\top(\kb_{i\alpha}-\kb_{i\beta})=\pb_1^\top(\kbb_{i\alpha}-\kbb_{i\beta})$. Thus, $\pb_1$ is exactly solving the same orthogonalized SVM problem as $\pb_2$.
%We will show this by proving that solution sets of two SVMs are equivalent. Specifically, we claim that solution $\pb^{\svm}$ of the original problem has to be orthogonal to $\W^\top\vstar$. Once $\pb^{\svm}$ is orthogonal to $\W^\top\vstar$, we observe that $(\pb^{\svm})^\top\W^\top\x_{it}=(\pb^{\svm})^\top\W^\top\cb_{it}$, thus, 
\end{proof}


\section{Contextual Dataset with Linear Values}\label{sec:linear data}




\noindent\textbf{Contextual Dataset Model:} We first describe the data distribution: Let $\X\in\R^{T\times d}$ be the input features and $Y\in\R$ be the associated label. For each input, we assume that the $T$ tokens are split into a label-relevant set $\Rc_{\X}\in[T]$ and a label-irrelevant set $\bar{\Rc}_{\X}=[T]-\Rc_{\X}$.


%Let $z\in\R$ be the label noise contributed by the irrelevant tokens. 

%and $\Dc_z$ be the irrelevant value distribution  to denote the value distribution over $\R^d\times \R^d$. Sample $\y\sim \Dc_y$ and $\z\sim \Dc_z$. 
%$\z$ can be viewed as a noise at the attention output. 
$\Rc_{\X}$ contains label-relevant features $\y\in\R^d$ and $\bar{\Rc}_{\X}$ contains label-irrelevant features $\z\in\R^d$. We will refer to $(\y,\z)$ as value vectors and assume them to be independent random variables with joint distribution denoted by $\Dc_{yz}$.
Each token $\x_t$ can be decomposed into a context vector $\cb_t$ and value vector $\y$ or $\z$ as follows.
\begin{align}
    \x_t=\cb_t+\begin{cases}\y\quad t\in \Rc_{\X}\\\z\quad t\in \bar{\Rc}_{\X}\end{cases}.\tag{CDM}\label{CDM}
\end{align}





As our core setting, we will consider a linear value model generated by a latent vector $\vstar$ and true label $Y$.
\begin{assumption}[Linear value model]\label{linass} Fix $\vstar\in\R^d$ and $\eps>0$. Let $\y=Y\cdot\vstar$ and $\z=Z\cdot\vstar$ where $Y,Z\in\R$ are independent random variables taking values $\pm1$ and $\pm \eps$ respectively.
\end{assumption}

Also denote the set of context vectors $\Cb=[\cb_1~\dots~\cb_T]^\top$. Since our primary focus is the role of attention, we will allow for arbitrary context vectors $\cb_t$. However, for cleaner exposition, we will make the following simplifying assumption on the label distribution.

\noindent\textbf{Interpretation:} Our contextual dataset admits the following interpretation. 
\begin{itemize}
    \item \textbf{(1a)} The context vectors $\Cb$ correspond to the key/query embeddings in the attention mechanism. They are used to locate relevant information in the input.
    \item \textbf{(1b)} Locating the relevant context will happen via the key-query weights $\W$ in self-attention or prompt vector $\pb$ in prompt-attention.
    \item \textbf{(2a)} The value vectors $(\y,\z)$ correspond to the value embeddings in the attention mechanism. $\y$ is used to infer the label whereas $\z$ serves as noise we aim to avoid.
    %from the relevant information.
    \item \textbf{(2b)} Obtaining the label prediction will happen via the value weights $\V$ or nonlinear head $\link{\cdot}$.
    %in self-attention or classifier head $\w$ in prompt-attention.
\end{itemize}

\noindent\textbf{Training Dataset:} Let $\Sc=(\X_i,Y_i)_{i=1}^n$ be the training dataset generated according to \eqref{CDM} where $(\X_i,Y_i)$ denote the $i^{th}$ input-label pair. Following above, let $\Cb_i\in\R^{T\times d}$ denote the context vector within $\X_i$ and $(\y_i,\z_i)$ denote the value vectors within $\X_i$ for $1\leq i\leq n$.

\noindent\textbf{Training Loss:} We are interested in optimizing our attention model over the dataset $\Sc$ using loss function $\ell$. While the context vectors are deterministic, value vectors $(\y,\z)$ are stochastic. To investigate implicit bias in contextual learning, we require a deterministic training loss. Thus, our training will take expectations over $(\y,\z)$.
\begin{align}%{ncols}
    \Lc(\bt)=\frac{1}{n}\sum_{i=1}^n \E_{\Dc_{yz}}[\ell(Y_i,f_{\bt}(\X_i))].\tag{ERM}\label{erm}
\end{align}
Above, $f$ is either self-attention $\fat$ (with parameters $\bt=[\W,\V]$) or prompt-attention $\fapt{}$. Since self-attention outputs $T$ tokens, when necessary, $f$ will use an additional classifier head that maps $T$ token into $1$.

%In case of self-attention, we note that $f$ will include  %Here, $\bt$ are the parameters of the attention model i.e.~$\bt=[\W,\V]$ or $\bt=[\pb,\w]$.
%We will initially focus on learning the context vectors, thus, $\bt=[\W,\V]$ and 
% As usual, we op
%\in\R^{T\times d}$ denote the input features and $Y_i$ denote the associated label. 

\subsection{Maximum Margin Context Separation}
Our key observation is treating relevant and irrelevant contexts as two separate classes. This allows us to use the implicit bias ideas to separate the resulting classes. Importantly, we need to do this for each input example. Namely, $\Cb_i=(\cb_{it})_{t=1}^T$ is treated as an input dataset. The $t^{th}$ token $\cb_{it}$ has label $r_{it}=1$ if $t\in\Rc_{\X_i}$ and $r_{it}=0$ otherwise. For this $i^{th}$ dataset, we are interested in maximum context margin that separates the single best relevant context from all irrelevant contexts. Formally, this is obtained by solving the following problem.
%For this $i^{th}$ dataset, the max-margin context separation can be obtained by solving the following problem.
\begin{align*}
    \min_{\pb,b}\tn{\pb}\quad\text{subject to}\quad \max_{t_1\in \Rc_{\X_i}}\min_{t_0\in \bar{\Rc}_{\X_i}}\pb^\top(\cb_{it_1}-\cb_{it_0})\geq 1\quad\text{for all}\quad t\in[T].%\label{max-margin-indiv}
\end{align*}
Above, note that the order of $\max$ and $\min$ can be swapped thanks to the minimax theorem. Additionally, for fixed $t_1$, $\min_{t_0\in \bar{\Rc}_{\X_i}}\pb^\top(\cb_{it_1}-\cb_{it_0})$ is simply attained at the nearest point to $\cb_{it_1}$ in the set $\{\cb_{it_0}\}_{t_0\in \bar{\Rc}_{\X_i}}$. 

In our case, we wish to find a solution which can separate $n$ samples each corresponding to a dataset $\Cb_i$. Thus, we can solve the following problem. 
\begin{align} %,(b_i)_{i=1}^n
    \pb^{\svm}=\arg\min_{\pb}\tn{\pb}\quad\text{subject to}\quad &m_i\geq 1\quad\text{for all}\quad i\in [n]\label{max-margin}\tag{SVM}\\
    \text{where}\quad &m_i=\max_{t_1\in \Rc_{\X_i}}\min_{t_0\in \bar{\Rc}_{\X_i}}\pb^\top(\cb_{it_1}-\cb_{it_0}).\nn
\end{align}
Here, let us refer to $m_i$ as the context margin of the $i$'th example. Then, above problem is optimizing for a vector $\pb$ which maximizes the smallest context margin over all input examples $(\X_i)_{i=1}^n$.

\begin{definition}[Relevant support contexts] Let $S_i\subset\Rc_{\X_i}$ be the relevant token indices that attains the margin $m_i$ for the solution of \eqref{max-margin}. We refer to $(\cb_{it})_{t\in S_i}$ as the support contexts of example $i$. Let $\Cb_{\svm}=(\cb_{it})_{t\in S_i, i\in [n]}$ be the set of all support contexts.
\end{definition}

\subsection{Implicit Bias of Attention}
The following assumption will be useful for cleaner exposition. We will later discuss how to relax it.
\begin{assumption} [Orthogonal Context-Value] For all $i\in [n],t\in[T]$, $\cb_{it}\perp\vstar$.
\end{assumption}
The following theorem formalizes our key insight on the implicit bias of the attention mechanism.

    

%prompt-attention model.
\begin{theorem} Suppose training set $\Sc$ is generated according to \eqref{CDM}. Consider \eqref{erm} with $f=\fapt{}$ and $\ell(\cdot)$ is either squared loss or logistic loss. Fix the classifier head $\vb=\vstar$ and only tune the prompt vector $\pb$ with iterations $\pb_{t+1}\gets \pb_t-\eta\Lcp(\pb_t)$ starting from some $\pb_0$. Then, gradient descent on prompt-attention converges to the max-margin context separator i.e.
    \begin{align}
        \lim_{t\rightarrow\infty} \frac{\pb_t}{\tn{\pb_t}}\rightarrow \frac{\pb^{\svm}}{\tn{\pb^{\svm}}}.
    \end{align}
\end{theorem}

Below, we state a more general theorem that explains the convergence of prompt-attention for general context-value when both $\vb,\pb$ are optimized.
\begin{theorem} Suppose training set $\Sc$ is generated according to \eqref{CDM}. Consider \eqref{erm} with $f=\fapt{}$ and $\ell(\cdot)$ is the logistic loss. Introduce the orthogonalizations $\vstar',(\Cb'_t)_{t=1}^T$ as follows:
\begin{itemize}
    \item $(\Cbp_i)_{i=1}^n$ are the context matrices associated to $(\X_i)_{i=1}^n$ after projecting $(\Cb_i)_{i=1}^n$ on the orthogonal complement of $\vstar$.
    \item $\pb^{\svm}$ is the solution to \eqref{max-margin} with orthogonalized contexts $\Cbp_i$ for $i\in[n]$.
    \item $\vstap$ is the projection of $\vstar$ onto the orthogonal span of all support contexts $\Cb_{\svm}$.
\end{itemize}
Given ridge regularization strengths $R_w,R_q$, define the regularized solution of prompt-attention as follows
\[
    \pb^\reg,\vb^\reg=\arg\min_{\pb,\vb}\Lcp(\pb,\V)\quad\text{subject to}\quad \tn{\pb}\leq R_q,\tn{\vb}\leq R_w.
\]
Then, as $R_q/R_w\rightarrow\infty$ and $R_w\rightarrow\infty$ we have that
\begin{align}
     \frac{\pb^\reg}{R_q}\rightarrow \frac{\pb^{\svm}}{\tn{\pb^{\svm}}}\quad\text{and}\quad \frac{\vb^\reg}{R_w}\rightarrow \frac{\vstap}{\tn{\vstap}}.
\end{align}
\end{theorem}


==> sec/exp_zz.tex <==
\section{Experiments}
\textbf{Dataset generation: } $(\X_i,y_i)_{i=1}^n$, where $\X_i\in\R^{T\times d}$ and each entry of $\X_i$ is i.i.d. randomly Gaussian distributed, and $y_i$'s are Rademacher variables. Let $\vb\in\R^d$ be an arbitrary unit-norm vector. Then we define the \emph{best} token of each input sequence $\X_i$ as follows:
\[
	best_i=\arg\max_{t\in[T]}y_i\cdot\vb^\top\x_{it}.
\]
Here we assume that for any $i\in[n]$, $\max_{t\in[T]}y_i\cdot\vb^\top\x_{it}>0$. Then given $best_i,i\in[n]$, we can get max-margin SVM solution $\ps$. 

During training, fix $\W,\vb$ and train prompt vector $\p$ only. Set $n=4,T=3,d=20$, and results are from $10$ runs.
\begin{itemize}
	\item $\W=\Iden$. Averaged results are shown in Figure~\ref{fig iden}.
	\item $\W=QK^\top$. Here instead of setting $\W$ to be identical, let $\W=QK^\top$ where $\W\in\R^{d\times d}$ and $Q,K\in\R^{d\times h}$, and $Q,K$ have random entries. Figure~\ref{fig h100} shows the result where $h=100$, while Figures~\ref{fig h10 succ},~\ref{fig h10 fail}\&\ref{fig h10 ps} show the results when setting $h=10<d$. 
\end{itemize}
Overall we can observe that when given nice initialization ($\p_{\text{init}}=\ps$), $\p$ will converge to $\ps$ through gradient descent. However, if $\p$ is randomly initialized, in our scenario, $h=10$ does not certainly converge.  

\begin{figure}
	\begin{minipage}{0.4\textwidth}
	\centering
	\includegraphics[scale=0.3]{exp/n4T3d20_identity_random_succeed(10_10).pdf}
	\caption{$\W=\Iden$}\label{fig iden}
	\end{minipage}
	\centering
	\begin{minipage}{0.4\textwidth}
	\includegraphics[scale=0.3]{exp/n4T3d20h100_random_succeed(10_10).pdf}
	\caption{$\W=QK^\top$, $h=100$}\label{fig h100}
	\end{minipage}
\end{figure}
\begin{figure}
	\begin{minipage}{0.33\textwidth}
	\centering
	\includegraphics[scale=0.25]{exp/n4T3d20h10_random_succeed(6_10).pdf}
	\caption{$h=10,succeed~(6/10)$}\label{fig h10 succ}
	\end{minipage}
	\centering
	\begin{minipage}{0.33\textwidth}
	\includegraphics[scale=0.25]{exp/n4T3d20h10_random_fail(4_10).pdf}
	\caption{$h=10,fail~(4/10)$}\label{fig h10 fail}
	\end{minipage}
	\begin{minipage}{0.33\textwidth}
	\includegraphics[scale=0.25]{exp/n4T3d20h10_psvm.pdf}
	\caption{$h=10,\p_\text{init}=\ps$}\label{fig h10 ps}
	\end{minipage}
\end{figure}
%\section*{Experimental setting}
%Parameters: $n,T,d$, $\Cb=\Nc(0,\Iden)\in\R^{T\times d}$, and relevant set $\Rc_{\X}\in[T]$
%
%\red{Q: Are $\Cb$ and $\Rc_{\X}$ fixed for all sequences $\X_1,\cdots,\X_n$? If consider self-attention, $\W\in\R^{T*d}$?}
%
%\grn{It is OK to fix $\Rc_{\X}$ e.g. you can make half good half bad. Initially you can also fix $\Cb$. However, as you see in \eqref{max-margin}, the solution will be different if you change $\Cb$. So we have to run experiments with different $\Cb$'s as well.}
%
%\grn{Below it clearly says $\W\in\R^{d\times v}$. Why do you think it is $\W\in\R^{T\times d}$? Note that $T$ would mismatch with $\X\W$. For self-attention, we will also use $v=1$ (at least initially) i.e. we simply have $\W=\w\in\R^d$. I will write down the self-attention statements tmr, so you can read it before starting the experiments.}
%
%
%\noindent\textbf{Date generation: } Assume $T=5$ and $\Rc_{\X}=\{1,3\}$, and $\X_1=[\cb_1\red{+\wstar},\cb_2-\wstar,\cb_3\red{+\wstar},\cb_4+\wstar,\cb_5+\wstar]$, $\X_2=[\cb_1\red{-\wstar},\cb_2-\wstar,\cb_3\red{-\wstar},\cb_4+\wstar,\cb_5-\wstar]$. 
%
%\grn{As I explained in the Slack, you might have to consider all labels/noises for each $\X$. This means generating 4 versions for each $\X$ ($y=\pm 1,z=\pm1$) unless you have a clear hypothesis on how it can be avoided. The idea is symmetrizing the dataset over the label so that we can isolate the role of context. If you check my code, you see that I create 8 versions ($\pm 1$ for 3 contexts). I am saying you just do 4 versions ($\pm 1$ for relevant and irrelevant contexts).}
%
%
%\noindent\textbf{Remarks.} (1) $\cb_1,\cdots,\cb_T$ are the same for all $\X_1,\cdots \X_n$, which means input space $\X\in\Xc\subset\R^{T\times d}$ is finite. (2) $\X_1$ corresponds to label $y=+1$ and $\X_2$ corresponds to label $y=-1$, which means that all the relevant positions have the same label in a sequence, and irrelevant output can be either $-1$ or $1$.
%
%Now assume what I claim above is correct and if consider multi-classification problem, there are the data generation versions as I understand.
%
%\begin{itemize}
%	\item Let $\W\in\R^{d\times v}$ where $v=\text{\# of classes}$. Then set $v$ orthogonal vector as labels and following the same data generation as above. \grn{I need to think more on this. So far, this setting is always binary classification however there can be multiple contexts. Also $\W$ is for self-attention, let us make sure prompt-attention works as expected first and we can discuss self-attn a bit later.}
%	\item Or we can keep using $v=1$, but make sure $|\Rc_{\X}|\geq\text{\# of classes}$. Then label of a sequence can be determined by vector $[y_1,y_3]^\top$ (if assuming $\Rc_{\X}=\{1,3\}$).
%\end{itemize}
%


==> sec/joint_fig.tex <==
    \begin{figure}[t]
    \centering
    % \hspace{-10pt}
    % \subfigure[The role of loss function]{
    %     \includegraphics[width=.33\columnwidth]{fig/diff_loss_func.pdf}
    %     \label{fig2:loss:sen}
        
    % }%\caption{Global convergence}
    \hspace{-15pt}
    \subfigure[All inputs are support vectors]{
        \includegraphics[width=.32\columnwidth, trim={0 -0.5cm 0 0}]{fig/joint_tight_converge.pdf}
        \label{fig2:allsvm}
    }
    %\caption{Convergence to global and local optima}
    \hspace{-5pt}
    \subfigure[(0.5,1.5) is not a support vector]{
        \includegraphics[width=.32\columnwidth, trim={0 -0.5cm 0 0}]{fig/joint_relax_converge.pdf}
        \label{fig2:nosvm}
    }
    \hspace{-10pt}
    \subfigure[Probability evolutions in \textbf{(a)}]{
        \includegraphics[width=.34\columnwidth, trim={0 .7cm 0 0}]{fig/joint_tight_converge_probs.pdf}
        \label{fig2:prob}
    }
    \vspace{-2mm}
    \caption{
        % \textbf{(a)} Global convergence of $\pb$ with different loss functions and scores. 
        \textbf{(a)} and \textbf{(b)} Joint convergence of attention weights $\pb$ ({\color{red} \footnotesize{--->---}}) and classifier head $\vb$ ({\color{blue} \footnotesize{--->---}}) to max-margin directions. \textbf{(c)} Averaged softmax probability evolution of optimal tokens and logistic probability evolution of output in \textbf{(a)}.}
    \label{fig:joint_fig}\vspace{-8pt}
    \end{figure}

==> sec/main_fig.tex <==
\begin{figure}[t]
\centering
\hspace{-10pt}
\subfigure[Global convergence]{
    \includegraphics[width=.33\columnwidth]{fig/global_converge.pdf}
    \label{fig:global}
    
}%\caption{Global convergence}
\hspace{-10pt}
\subfigure[Global and local optimal directions]{
    \includegraphics[width=.33\columnwidth]{fig/local_converge.pdf}
    \label{fig:local}
    
}%\caption{Convergence to global and local optima}
\hspace{-10pt}
\subfigure[Multiple inputs]{
    \includegraphics[width=.33\columnwidth]{fig/multi_converge.pdf}
    \label{fig:joint global}
}
\vspace{-2mm}
\caption{The convergence behavior of the gradient descent on the attention weights $\pb$ using the logistic loss in \eqref{lin det losss}. The arrows ({\color{gray} \footnotesize{--->---}}) represent trajectories from different initializations. Here, ({\color{red}-~-~-}) and ({\color{blue}-~-~-}) denote the global and local max-margin solutions. $\gamma$ denotes the \emph{score} of a token per Definition \ref{score def}. Discussion is provided under Theorem \ref{conv:gd:global}.}
\label{fig:main_fig}\vspace{-5pt}
\end{figure}
%the global and local convergence of $\pb$ ({\color{gray} \footnotesize{--->---}}) for fixed $\vb$ to the global ({\color{red}-~-~-}) and local ({\color{blue}-~-~-}) max-margin solutions

==> sec/real_data_fig.tex <==
\begin{figure}
\begin{minipage}{7cm}
    \centering
    \subfigure[Input image]{
        \includegraphics[width=.3\columnwidth]{exp/real_data/image.pdf}
        \label{fig:real_image}
        
        
    }
    \subfigure[epoch 0]{
        \includegraphics[width=.3\columnwidth]{exp/real_data/attention_0.pdf}
        \label{fig:real_image_0}
    }
        \subfigure[epoch 100]{
        \includegraphics[width=.3\columnwidth]{exp/real_data/attention_100.pdf}
        \label{fig:real_image_100}
    }
    % \subfigure[sparsity]{
    %     \includegraphics[width=.43\columnwidth]{exp/real_data/sparsity_norm.pdf}
    %     \label{fig:sparsity}
    % }
    
            \subfigure[epoch 200]{
        \includegraphics[width=.3\columnwidth]{exp/real_data/attention_200.pdf}
        \label{fig:real_image_200}
    }
            \subfigure[epoch 300]{
        \includegraphics[width=.3\columnwidth]{exp/real_data/attention_300.pdf}
        \label{fig:real_image_300}
    }
                \subfigure[epoch 400]{
        \includegraphics[width=.3\columnwidth]{exp/real_data/attention_400.pdf}
        \label{fig:real_image_400}
    }
    
        \caption{Illustration of how attention weights of \texttt{[CLS]} token progressive change during training in the transformer model for a given input image \ref{fig:real_image}. We analyze the average value derived from all attention heads within the last layer of the model.}
        
    \label{fig:att_map}
    \end{minipage}
    \hspace{5pt}
\begin{minipage}{7cm}
    \centering
    \subfigure[]{
        \includegraphics[width=\columnwidth]{exp/real_data/sparsity_norm.pdf}
        \label{fig:sparsity}
    }
 %   \subfigure[weight norm]{
%      \includegraphics[width=.33\columnwidth]{exp/real_data/weight_norm.pdf}
%     \label{fig:weight}
% }
        \caption{The effective sparsity quantifies the sparsity level of the softmax probability vector. More spare vector(smaller value) means a few key elements receive significantly higher attention, while the majority of the elements receive minimal attention. Norm of attention weight are defined as the L2 norm of the key-query matrix $W=WK WQ^T$ over time.}
    \label{fig:att_sparsity}
\end{minipage}
\end{figure}

==> sec/self_attention.tex <==
\section{Implicit Bias of Training on Self-Attention Output}

\red{[\textbf{Basic deliverable for self-attention:} If $\x_1$ admits a constant projection ($\W=\W_Q\W_K^\top$ with constant $\W_Q^\top \x_1$), then, the result is same as rank-1 $\W$ convergence. Otherwise, even with a dataset of two inputs, the optimal solution is actually rank-2 and this solution does not necessarily map $\W^\top\x_1$ to the $\x_{\svm}$.]}

% and denoting the first token by $\x_i:=\x_{i1}$,
%we set $\hat{Y}=\V^\top\X^\top\sft{\X\W^\top\x_1}$ and 
% Since self-attention outputs multiple tokens, we will allow for multiple labels per input where 
%dataset $(X_i,Y_i)_{i=1}^n$,
In this section we consider the self-attention model \eqref{satt}. Let us first investigate the scenario where we use the first token output to make a classification decision. That is, given a input-label distribution $(X,Y)\sim\Dc$, denoting the first token as $\x_1$, we consider the following classification problem:
\begin{align}
\Lc(\W)=\E_{\Dc}\left[\sum_{i=1}^n \ell(Y,\vb^\top\X^\top\sft{\X\W^\top\x_1})\right].\label{satt loss}
%\frac{1}{n}\sum_{i=1}^n \ell(Y_i,\V^\top\X_i^\top\sft{\X_i\W^\top\fb_{i}}).\label{satt loss}
\end{align}
Recalling \eqref{patt}, two key differences are (i) we are optimizing a matrix $\W$ and (ii) unlike prompt or \cls token $\pb$, the first token $\fb_i$ is a feature that varies with $\X_i$. Our investigation will uncover an implicit bias phenomena under a contextual dataset described next.

\begin{definition}[Multi-context Input] \label{def:multi_context} Fix $\wstar\in\R^d$ and $\Cb\in\R^{T\times d}$ and suppose $\Cb\wstar=0$. Let $(\eps_t)_{t=1}^T$ be Rademacher random variables. Consider the input distribution $\X$ with $\x_t=\eps_t\cdot\wstar+\cb_t$ for $t\in[T]$.
\begin{itemize}
    \item \textbf{Single-label setting:} The label associated to $\X$ is $Y=\eps_1$.
    \item \textbf{Multi-label setting:} Let $K\in [T]$. The label associated to $\X$ is $Y=[\eps_1,\eps_2,\dots,\eps_K]$.
\end{itemize}
%\noindent\textbf{(a) Single-label setting:} The label associated to $\X$ is $Y=\eps_1$.
%\noindent\textbf{(b) Multi-label setting:} The label associated to $\X$ is $Y=\eps_1$.
\end{definition}
%Let $\Sc=(\X_i,Y_i)_{i=1}^n$ is a dataset generated from the above distribution. We consider the following classification problem:
\begin{theorem}[Single-label] Consider Definition \ref{def:multi_context} with single-label setting. Let $\Sc_R$ be the set of $\W$ obeying $\W^\top\wstar=\W\wstar=0$ and $\tf{\W}\leq R$. Recalling \eqref{satt loss}, set $\vb=\wstar$ and $\W_R=\arg\min_{\W\in \Sc_R}\Lc(\W)$. We have that
\[
\lim_{R\rightarrow\infty}\frac{\W_R}{R}=\frac{\W^\svm}{\tf{\W^\svm}},
\]
where $\W^\svm=\cb_1\pb_{\svm}^\top$ is a rank-$1$ matrix and $\pb_{\svm}$ is the solution of the max-margin SVM on contexts $(\cb_t)_{t=1}^T$,
\[
\min_{\pb} \tn{\pb}\quad \text{subject to}\quad \pb^\top (\cb_1-\cb_t)\geq 1\quad\text{for all}\quad t\in[T]-\{1\}.
\]
%Additionally, $\W^{\svm}=$
\end{theorem}
\subsection{Implicit Bias of Multi-label Learning}
In this section, we investigate the scenario where the goal is training a $\W$ that can predict multiple labels. Let $Y\in\R^K$ and consider the following multi-label learning problem where $k^{th}$ tokens output predicts $k^{th}$ label $Y^{(k)}$ for $k\in[K]$:
\begin{align}
\Lc_K(\W)=\E_{\Dc}\left[\sum_{i=1}^n \sum_{k=1}^K\ell(Y^{(k)},\vb^\top\X^\top\sft{\X\W^\top\x_k})\right].\label{satt loss2}
\end{align}

\begin{theorem}\red{[TO BE PROVEN]} Consider Definition \ref{def:multi_context} with multi-label setting. Let $\Sc_R$ be the set of $\W$ obeying $\W^\top\wstar=\W\wstar=0$ and $\tf{\W}\leq R$. Recalling \eqref{satt loss2}, set $\vb=\wstar$ and $\W_R=\arg\min_{\W\in\Sc_R}\Lc_K(\W)$. We have that
    \[
    \lim_{R\rightarrow\infty}\frac{\W_R}{R}=\frac{\W^\svm}{\tf{\W^\svm}},
    \]
    where $\W^\svm$ is \red{a matrix with rank at most $K$} obtained as the solution of the max-margin SVM on $(\cb_t)_{t=1}^T$ as follows,
    \[
    \min_{\W} \tf{\W}\quad \text{subject to}\quad \cb_k^\top \W(\cb_k-\cb_t)\geq 1\quad\text{for all}\quad k\in[K],t\in[T]-\{k\}.
    \]%\red{\|\W\|_{\star}}\quad(\text{not}~\tf{\W})
    %Additionally, $\W^{\svm}=$
    %\red{with minimum nuclear norm} 
    \end{theorem}

\begin{comment}
\newpage
\noindent\textbf{\red{(NEWPAGE) Dataset model and TODOs:}}
\begin{itemize}
    \item Contains multiple contexts and corresponding labels.
    \item Only tune the prompt vectors and not the class labels
    \item Allow nonlinear head: You can abstract out the whole TF as \emph{nonlinear follow-up layers}
    \item Implicit bias: Does softmax-prompt-tuning converge to (some) max-margin of the correct context?
    \item Is prompt-vector eventually orthogonal to its corresponding label?
    \item Joint implicit bias: Head vector converges to $\wstar'$ (orth to $\qstar$) whereas prompt converges to $\qstar'$ which is orthogonal to $\wstar$ and max-margin to remaining contexts. 
\end{itemize}
\end{comment}
